Calibrate: Frequency Estimation and Heavy Hitter Identification with Local Differential Privacy via Incorporating Prior Knowledge

Estimating frequencies of certain items among a population is a basic step in data analytics, which enables more advanced data analytics (e.g., heavy hitter identification, frequent pattern mining), client software optimization, and detecting unwanted or malicious hijacking of user settings in browsers. Frequency estimation and heavy hitter identification with local differential privacy (LDP) protect user privacy as well as the data collector. Existing LDP algorithms cannot leverage 1) prior knowledge about the noise in the estimated item frequencies and 2) prior knowledge about the true item frequencies. As a result, they achieve suboptimal performance in practice. In this work, we aim to design LDP algorithms that can leverage such prior knowledge. Specifically, we design ${Calibrate}$ to incorporate the prior knowledge via statistical inference. ${Calibrate}$ can be appended to an existing LDP algorithm to reduce its estimation errors. We model the prior knowledge about the noise and the true item frequencies as two probability distributions, respectively. Given the two probability distributions and an estimated frequency of an item produced by an existing LDP algorithm, our ${Calibrate}$ computes the conditional probability distribution of the item's frequency and uses the mean of the conditional probability distribution as the calibrated frequency for the item. It is challenging to estimate the two probability distributions due to data sparsity. We address the challenge via integrating techniques from statistics and machine learning. Our empirical results on two real-world datasets show that ${Calibrate}$ significantly outperforms state-of-the-art LDP algorithms for frequency estimation and heavy hitter identification.

==> itemset.tex <==
\section{Application of $Calibrate$ to Item Set}
\label{sec:itemset}
In this section, we demonstrate that $Calibrate$ can also be used to improve frequency estimation in the scenario where each user has a set of items instead of one item. 
Such set-valued data occurs frequently in real-world scenarios, such as webpages visited by users~\cite{Kosarakdata}, web search queries~\cite{aolsearchdata}, and emojis typed by users~\cite{AppLDP17}.  
%A natural question is how to collect those information privately.
%Thus, how to privately estimate each items's frequency accurately when applying LDP over set-valued data is important.
To privately estimate item frequencies in these scenarios, LDP algorithms over set-valued data have been proposed recently. For example, Qin et al.~\cite{QinHeavyHitterCCS16} proposed a padding and sampling based algorithm. Apple~\cite{AppLDP17}  deployed a similar LDP algorithm on iOS system to estimate the frequencies of emojis typed by users. Microsoft~\cite{ding2017collecting} has also deployed an algorithm in Windows 10 Update to collect telemetry over millions of devices repeatedly.
%Specifically, each user possess an item set of emoji. The system first apply random LDP algorithm to each item and then randomly sample one private item when number of items reach the limit and sends the sampled private item to the server. 
Similar to the LDP algorithms for single-item users, these algorithms for set-valued data did not consider the prior knowledge about the noise and true item frequencies. Our $Calibrate$ framework can be applied to improve the estimation accuracy of these algorithms. 
%For example, our experiment show that our Calibrate framework can decrease the estimation error by an order of magnitude in real world dataset. 
%Similarly, existing algorithm don't consider the prior distribution information of items which incur high estimation error. Our Calibrate framework can simply apply to existing algorithm and significantly improve the estimation accuracy.


\myparatight{LDP algorithms for set-valued data}
Qin et al.~\cite{QinHeavyHitterCCS16} proposed LDPMiner, a two-phase algorithm to estimate item frequencies of heavy hitters for set-valued data. 
The Phase I of LDPMiner estimates frequencies of all items via a sampling randomizer algorithm. Since our work focuses on frequency estimation of all items, we use the Phase I of LDPMiner. Specifically, the algorithm first fixes each user to have $l$ items. If a user has less than $l$ items, then the algorithm randomly pads dummy items for the user, otherwise the algorithm randomly samples $l$ items from the user's true items. The dummy items are not considered by the data collector when estimating frequencies.  Then, the algorithm samples one item from the $l$ items for each user and applies an existing LDP algorithm for single-item data on the sampled item. The server multiplies each item's frequency by $l$ to get unbiased estimations as the final output. Qin et al.~\cite{QinHeavyHitterCCS16} explored RAPPOR~\cite{Erlingsson:2014} and Succinct Histogram (SH)~\cite{BassilySuccinctHistograms15} as the LDP algorithm for single-item data. We consider OUE~\cite{Ninghui:2017} since it achieves state-of-the-art performance for single-item data.  

%  RAPPOR and sampling Succinct histogram (SH)~\cite{BassilySuccinctHistograms15} and show that they outperform simply apply RAPPOR and SH via split privacy budget. We replace RAPPOR and SH with OUE and OLH and get the state-of-the-art LDP algorithm.
%The main idea of sampling OUE is padding and sampling. Specifically, we first fix each user has $l$ items by padding fake items or randomly delete some items for each user. 
%Then, we randomly sample one item for each user and apply OUE or OLH directly for each user. After receiving perturbed items from users, the server can estimate the frequency for each items which is the same with OUE or OLH. Then, the server multiply each item's frequency by $l$ to get unbiased estimation as the final output. 

\myparatight{Estimating $p_s$, $p_f$, and $p_{\hat{f}}$}
When $l$ is large enough such that we only pad dummy items to users, the noise of the sampling algorithm with OUE still follows a Gaussian distribution. In particular, since the server multiplies the frequency produced by OUE by $l$, the Gaussian distribution still has zero mean but the variance is  $l^2$ times of that in the Gaussian noise distribution of OUE.  When $l$ is not large enough, some users' true items get truncated. As a result, the noise does not exactly follow a Gaussian distribution. However, in practice, $l$ is often set to be large (e.g., 90-percentile of item-set size of all users recommended by~\cite{QinHeavyHitterCCS16}) in order to achieve good estimation accuracies. Therefore, we still use a Gaussian distribution to approximate the noise. Once we know the noise distribution and the estimated item frequencies, we can estimate $p_f$  and $p_{\hat{f}}$ using the techniques we discussed in Section~\ref{estimatepf}.


%As we have analized before, the noise for OUE and OLH is zero-mean Gaussian distribution. When estimate the true frequency, it is multiplied by $l$. Because a gaussian random variable multiplied by a constant $a$, then, it is still a gaussian distribution. The mean and variance become $l$ and $l^2$ times of origin mean and variance respectively. 
%However, because some of user has more than $l$ items, when we truncate items for those users, we would lost those items for those users. This will makes the mean of noise distribution non-zero. However, when we set $l$ to a relative large number, such as 90-percentile of item size of all users used in~\cite{QinHeavyHitterCCS16}. It has relatively small influence on the mean shift of noise distribution. Thus, we still can assume the noise is zero-mean gaussian distribution.
%$p_f$  and $p_{\hat{f}}$ are determined in the same way as previous, please refer to Section 3.3. 
\myparatight{Experimental result}
Like previous study~\cite{QinHeavyHitterCCS16}, we use the {Kosarak} dataset~\cite{Kosarakdata} for evaluation. In the dataset, each user has clicked a set of webpages and we aim to estimate frequency for each webpage. We set $l$ to the 90-percentile of all users' item-set size, as suggested by~\cite{QinHeavyHitterCCS16}. Moreover, we assume the distribution family of the true item frequencies is already known, i.e., power-law distribution for the {Kosarak} dataset.
 Figure~\ref{itemset} shows the estimation errors as we increase the privacy budget. As we can see, our $Calibrate$ can reduce the estimation errors by orders of magnitude. 


%\subsection{Problem Description}
%Suppose we have $d$ items (indexed by $\{1,2,\cdots,d\}$) and $n$ users. Each user $u_i$ has $l_i$ items and we use $\mathbf{I}_i$ to denote corresponding item set. Directly applying existing LDP algorithm to item set face some challenges since each user has different number of items. For example, when applying OUE, we can set encoding vector $\mathbf{X}[i]=1$ if user has item $i$, otherwise, set it to $0$. Then, for each user, it's encoding vector has $l_i$ nonzero value, that is, the sensitivity is $2l_i$. Thus, we have the following perturbing method:
%\begin{align}
%\label{oueperturbitemset}
%\text{Pr}(\mathbf{Y}[i]=1)=\left \{ 
%\begin{aligned}
%p=&\frac{1}{2}, \text{ if }\mathbf{X}[i]=1 \\
%q=&\frac{1}{1+e^{\frac{\epsilon}{2l_i}}}, \text{ if }\mathbf{X}[i]=0 
%\end{aligned}
%\right.
%\end{align}
%Thus, as we can see, for each user, the value $q$ is different due to its different sensitivity which makes it difficulty to estimate the frequency of items. As pointed in~\cite{QinHeavyHitterCCS16}, a method is to have a fixed $l$ for each user. 
%If a user has less than $l$ items, then, we can padding fake items. Correspondingly, if a user has more than $l$ items, we can truncate the user's items to $l$, that is, randomly delete some items for that user. Based on this, Qin et al.~\cite{QinHeavyHitterCCS16} propose a sampling based method to estimate the frequency of items over set-valued data. Apple~\cite{AppLDP17} uses a similar sampling based LDP system to collect emoji typed by users.  
%Specifically, Qin et al.~\cite{QinHeavyHitterCCS16} proposed sampling randomizer in which each user randomly choose an items and reports it rather than report all items. When estimating items' frequency, we multiply estimated frequency by $l$ to get an unbiased estimation. 

%\subsection{Existing Algorithm}
%In this section, we have a detail description of the sampling OUE since sampling OLH have the same accuracy with sampling OUE. We omit sampling OLH for simplicity. 
%For each user,  Then, we randomly sample an item from $l$ items for each user and then apply random LDP algorithm and sends perturbed result to the server. After receiving those result, server can estimate the frequency of each items and then multiply frequency by $l$ to get an unbiased estimation. Then, we can apply our Calibrate framework to calibrate estimated frequency. 
%\subsection{Noise Distribution Analysis}

%\subsection{Experiment Result}
%\myparatight{Real-world dataset (Kosarak)}: 

%\myparatight{Parameter Setting} 

%\myparatight{Compared Method} 

%\myparatight{Result} 

\begin{figure}[!t]
%\vspace{-2mm}
\centering
%\subfloat[Basic]
{\includegraphics[width=0.450 \textwidth]{figs/square/itemset.pdf}}
\caption{Estimation errors for set-valued data on the Kosarak dataset.}
\label{itemset}
\end{figure}




==> method.tex <==
\section{Our Defense Framework}
We propose a two-phase framework MaLIAGuard to solve the inference-attack defense problems.
We first discuss how we solve the Inference-Attack Defense Problem I. 
Then, we introduce our solution for the Inference-Attack Defense Problem II.


\subsection{Inference-Attack Defense Problem I}
%Essentially, we aim to obtain a randomized noise addition mechanism $\mathcal{M}$ via solving the optimization problem in Equation~\ref{prb}. 
We consider four scenarios depending on whether the defender knows the prior probability distribution $\mathbf{p}$ and the classifier $C$ used by the attacker:
\begin{packeditemize}
\item {\bf Scenario I:} known $\mathbf{p}$ and known $C$.
\item {\bf Scenario II:} unknown $\mathbf{p}$ and known $C$. 
\item {\bf Scenario III:} known $\mathbf{p}$ and unknown $C$. 
\item {\bf Scenario IV:} unknown $\mathbf{p}$ and unknown $C$. 
\end{packeditemize} 

The defender could know $\mathbf{p}$ and $C$ if the defender is an \emph{insider} of the attacker. 
For instance, suppose a social media provider aims to infer private attribute values of its users.
The inferred attribute values can be leveraged to perform targeted advertisements, and thus increase revenues.  
In this example, the social media provider is treated as an attacker, 
and the social media's (former) employee could be a defender who develops a browser extension to help users protect their private attributes.
Such a defender knows the $\mathbf{p}$ and $C$ used by the attacker. 

When the prior probability distribution $\mathbf{p}$ is unknown, we find a $\mathcal{M}$ such that the privacy risk is within the budget for any $\mathbf{p}$. 
When the classifier $C$ is unknown, the defender uses publicly available data to learn a classifier $C_d$ and treats it as if it were the classifier used by the attacker. 
The attacker's classifier essentially captures the relationships between a user's public data 
and private attribute value. 
Once the defender learns a classifier $C_d$ that well captures such relationships, 
the defender can use it to approximate $C$.% in solving the optimization problem in  Equation~\ref{prb}.

Next, we discuss how we solve the Inference-Attack Defense Problem I (i.e., Equation~\ref{prb}) for the four scenarios. 

\subsubsection{Scenario I: known $\mathbf{p}$ and known $C$} 
The major challenge to solve the optimization problem in Equation~\ref{prb} is that the randomized noise addition mechanism $\mathcal{M}$, which is a probabilistic mapping between two vectors, has lots of parameters.  Suppose the public data has $n$ entries and each entry takes a binary value, then $\mathcal{M}$ is characterized by $2^{2n}$ parameters.  
To address the challenge, 
we propose a \emph{two-phase framework} to solve the optimization problem. 
In Phase I, we find the minimum noise $\mathbf{r}_i$ that makes the attacker's classifier $C$ predict attribute value $i$ for the user, where $i\in \{1,2,\cdots,m\}$.
In Phase II, we find a $\mathcal{M}$, which is a probability distribution over the $m$ discrete noises $\{\mathbf{r}_1, \mathbf{r}_2, \cdots, \mathbf{r}_m\}$,  to achieve a privacy risk within the budget $\alpha$ while minimizing the utility loss. Under our framework, $\mathcal{M}$ only has $m$ non-zero parameters. 

\myparatight{Phase I: finding $\mathbf{r}_i$} The user's public data is $\mathbf{x}$. Suppose we aim to add minimum noise $\mathbf{r}_i$ to $\mathbf{x}$, according to the specified noise-type-policy $\mathcal{P}$, 
such that the classifier $C$ infers the attribute value $i$ for the user. Formally, we model finding such  $\mathbf{r}_i$ as solving the following optimization problem:
\begin{align}
& \mathbf{r}_i = \argmin_{\mathbf{r}} ||\mathbf{r}||_0 \nonumber \\
\label{findr}
\text{subject to } & C(\mathbf{x+r})=i.
\end{align}

\begin{algorithm}[t]
\caption{Policy-Aware Noise Finding Algorithm}
\begin{algorithmic}[1]
\REQUIRE Public data $\textbf{x}$, classifier $\textbf{C}$, noise-type-policy $\mathcal{P}$, target attribute value $i$, and step size $\tau$. \\
\ENSURE  Noise $\textbf{r}_i$. \\
    %Initialize $\textbf{x}_{0}=\textbf{x}$ \\
    Initialize $t=0,\overline{\textbf{x}}=\textbf{x}$. \;
%\noindent \textbf{Process:}
%\PROCESS ~~\\
    %\WHILE { $\sum_{u\in V}|\hat{{p}}_u^{(t)} - \hat{{p}}_u^{(t-1)}| \geq \delta$ and $t \leq T$} \;
	%\IF{$\textbf{C}(\textbf{x})==i$} \RETURN $\textbf{0}$ \ENDIF \\
	
	\WHILE { $\textbf{C}(\overline{\textbf{x}}) \neq i$ and $t \leq \text{maxiter}$} \;
	\STATE //Find the entry to be modified. \;
	\IF{$\mathcal{P}==Add\_New$} \;
	
	\STATE $e_{inc}=\argmax_{j} \{\frac{\partial \textbf{C}_{i}(\overline{\mathbf{x}})}{\partial \mathbf{x}_j}| \mathbf{x}_j=0\} $ \;
	\ENDIF\;
	
	\IF{$\mathcal{P}==Modify\_Exist$} \;
	\STATE $e_{inc}=\argmax_{j} \{(1-\overline{\textbf{x}}_j) \frac{\partial \textbf{C}_{i}(\overline{\mathbf{x}})}{\partial \mathbf{x}_j}| \mathbf{x}_j \neq 0\}$ \;
	
	%(\textbf{1}-\overline{\textbf{x}})\times \triangledown \textbf{C}_{i}$ \\
	\STATE $e_{dec}=\argmax_{j} \{-\overline{\textbf{x}}_j \frac{\partial \textbf{C}_{i}(\overline{\mathbf{x}})}{\partial \mathbf{x}_j}| \mathbf{x}_j \neq 0\}$ \;
	\ENDIF \\
	
	\IF{$\mathcal{P}==Modify\_Add$} \;
	\STATE $e_{inc}=\argmax_{j} \{(1-\overline{\textbf{x}}_j) \frac{\partial \textbf{C}_{i}(\overline{\mathbf{x}})}{\partial \mathbf{x}_j}\}$ \;
	
	%(\textbf{1}-\overline{\textbf{x}})\times \triangledown \textbf{C}_{i}$ \\
	\STATE $e_{dec}=\argmax_{j} \{-\overline{\textbf{x}}_j \frac{\partial \textbf{C}_{i}(\overline{\mathbf{x}})}{\partial \mathbf{x}_j}\}$ \;
	\ENDIF \\



	\STATE //Modify the entry $\overline{\textbf{x}}_{e_{inc}}$ or $\overline{\textbf{x}}_{e_{dec}}$ depending on which one is more beneficial. \;
	\STATE $v_{inc}=(\textbf{1}-\overline{\textbf{x}}_{e_{inc}}) \frac{\partial \textbf{C}_{i}(\overline{\mathbf{x}})}{\partial \mathbf{x}_{e_{inc}}}$ \;
	\STATE $v_{dec}=-\overline{\textbf{x}}_{e_{dec}} \frac{\partial \textbf{C}_{i}(\overline{\mathbf{x}})}{\partial \mathbf{x}_{e_{dec}}}$ \;
	\IF {$\mathcal{P}==Add\_New$ or $v_{inc} \geq  v_{dec}$} \;
	%\WHILE { $ \frac{\partial \textbf{C}_{i}(\overline{\mathbf{x}})}{\partial \mathbf{x}_{e_{inc}}} > 0 $ and $\overline{\textbf{x}}_{e_{inc}}<1$} \;
	
	\STATE $\overline{\textbf{x}}_{e_{inc}} = clip(\overline{\textbf{x}}_{e_{inc}}+ \tau)$ \;
	\label{clip1}
	%\ENDWHILE \;
	\ELSE 
	%\WHILE { $\frac{\partial \textbf{C}_{i}(\overline{\mathbf{x}})}{\partial \mathbf{x}_{e_{dec}}} < 0 $ and $\overline{\textbf{x}}_{e_{dec}}>0$} \;
	
	\STATE $\overline{\textbf{x}}_{e_{dec}} = clip(\overline{\textbf{x}}_{e_{dec}} - \tau)$ \;
	\label{clip2}
	%\ENDWHILE \;
	\ENDIF \;
	\STATE $t=t+1$ \;
	\ENDWHILE \;
%	
	\RETURN $\overline{\textbf{x}}-\textbf{x}$. \;

    % \WHILE { $\textbf{F}(\textbf{x}_{i}) \neq l_{t}$ and $i \leq maxiter$} \;
	% \STATE $i_{max1}=\argmax_{j} (\textbf{1}-\textbf{x}_{i})\times \triangledown \textbf{F}_{l_{t}}$ \\
	% \STATE $value=(\textbf{1}-\textbf{x}_{i}) \times \textbf{F}_{l_{t}}[i_{max1}]$ \\	
	% \STATE $i_{decrease}=\argmax_{j} \textbf{x}_{i} \times (\textbf{-1}) \times \triangledown \textbf{F}_{l_{t}}$ \\
	% \IF {$value \geq  \textbf{x}_{i} \times (-\textbf{1})\times \triangledown \textbf{F}_{l_{t}}[i_{decrease}]$} \;
	% %\STATE $i_{max}=i_{max1}$ \\
	% \STATE $\textbf{r}_{i}[i_{max1}]$=1.0 \\
	% \ELSE \;
	% %\STATE $i_{max}=i_{max2}$ \\
	% \STATE $\textbf{r}_{i}[i_{max2}]$=0.0 \\
	% \ENDIF \\
	% \STATE $\textbf{x}_{i+1}=\textbf{x}_{i}+\textbf{r}_{i}$ \\
	% \STATE $i=i+1$ \\
    % \ENDWHILE \\
    % \RETURN $\widehat{\textbf{r}}=\sum_{i}\textbf{r}_{i}$. \\
\end{algorithmic}
\label{algorithm2}
\end{algorithm}

Our formulation of finding $\mathbf{r}_i$ is closely related to \emph{adversarial machine learning}. 
In particular, finding $\mathbf{r}_i$ can be viewed as an \emph{evasion attack}~\cite{barreno2006can,laskov2014practical,Goodfellow:ICLR:14b,Papernot:arxiv:16Limitation,XuEvasionMalware,sharif2016accessorize} to the classifier $C$. 
However, existing evasion attack algorithms (e.g.,~\cite{Goodfellow:ICLR:14b,Papernot:arxiv:16Limitation}) are insufficient to solve $\mathbf{r}_i$ in our problem. The key reason is that they do not consider the noise-type-policy, which specifies the types of noises that can be added. 
We note that evasion attacks to machine learning are generally treated as offensive techniques, but our work demonstrates that evasion attacks can also be used as defensive techniques, e.g., defending against MaLIA. 

Papernot et al.~\cite{Papernot:arxiv:16Limitation} recently proposed a \emph{Jacobian-based Saliency Map  Attack} (JSMA) to deep neural networks.  They demonstrated that JSMA can find small noises (measured by $L_0$ norm) to evade a deep neural network.  Their algorithm iteratively adds noise to an example ($\mathbf{x}$ in our case) until the classifier $C$ predicts $i$ as its label or the maximum number of iterations is reached. 
In each iteration, the algorithm picks  one or two entries of $\mathbf{x}$ based on saliency map, and then increase or decrease the entries by a {constant} value. 

We also design our algorithm based on saliency map. However, our algorithm is different from JSMA in two aspects.  First, our algorithm incorporates the noise-type-policy, while theirs does not. The major reason is that their algorithm is not developed for preserving privacy, so they do not have noise-type-policy as an input. 
Second, in their algorithm, all the modified entries of  $\mathbf{x}$ are either increased or decreased. In our algorithm, some entries can be increased while other entries can be decreased. %Third, in each iteration, our algorithm adds or subtracts a varying value to the selected entry of $\mathbf{x}$, instead of a constant value. 
As we will demonstrate in our experiments, our algorithm can find smaller noises than JSMA.


Algorithm~\ref{algorithm2} shows our algorithm to find $\mathbf{r}_i$. We call our algorithm \emph{\underline{P}olicy-\underline{A}ware \underline{N}oise Fin\underline{d}ing \underline{A}lgorithm (PANDA)}. Roughly speaking, in each iteration, based on the noise-type-policy and saliency map, we find the entry of $\mathbf{x}$, by increasing or decreasing which the noisy public data could most likely move towards the class $i$. Then, we modify the entry by $\tau$, which is a parameter in our algorithm. We will discuss setting $\tau$ in our experiments. The operation $clip(y)$ at lines~\ref{clip1} and~\ref{clip2} normalizes the value $y$ to be in [0,1], i.e., $clip(y)=1$ if $y>1$,  $clip(y)=0$ if $y<0$, and $clip(y)=y$ otherwise. 
We note that, for the noise-type-policy Modify\_Add, our algorithm can always find a solution $\mathbf{r}_i$, because this policy allows us to explore each possible public data vector. However, for the policies Modify\_Exist and Add\_New, there might exist no solution $\mathbf{r}_i$ for Equation~\ref{findr}. In such cases, we will automatically extend to the Modify\_Add policy. 



\myparatight{Phase II: finding $\mathcal{M}^*$} In our framework, after the defender solves $\{\mathbf{r}_1, \mathbf{r}_2, \cdots, \mathbf{r}_m\}$, the defender randomly samples one of them with a certain probability and adds it to the user's public data $\mathbf{x}$.
Therefore, in our framework, the randomized noise addition mechanism $\mathcal{M}$ is a probability distribution over $\{\mathbf{r}_1, \mathbf{r}_2, \cdots, \mathbf{r}_m\}$, where $\mathcal{M}_i$ is the probability that the defender adds $\mathbf{r}_i$ to $\mathbf{x}$. 
Since $q_i=\text{Pr}(C(\mathbf{x+r})=i)$ and $C(\mathbf{x+r}_i)=i$, we have $q_i=\mathcal{M}_i$, where $i\in \{1,2,\cdots,m\}$. Therefore, we can transform the optimization problem in Equation~\ref{prb} as follows:
\begin{align}
%\textbf{Privacy-utility tradeoff } & \textbf{with a privacy-risk budget:} \nonumber \\
\mathcal{M}^*=&\argmin_{\mathcal{M}} \sum_{i=1}^m \mathcal{M}_i ||\mathbf{r}_i||_0 \nonumber \\
\label{prb-1}
\text{subject to }  & KL(\mathbf{p}||\mathcal{M}) \leq \alpha \nonumber \\
& \mathcal{M}_i > 0, \forall i\in \{1,2,\cdots,m\} \nonumber \\
& \sum_{i=1}^m \mathcal{M}_i = 1.
\end{align}
Next, we discuss our method to solve the above optimization problem. 
First, according to the definition of convex optimization problem~\cite{convexOptimization}, we can show that the above optimization problem is convex, so $\mathcal{M}^*$ is a global minimum.  Therefore, according to the \emph{Karush-Kuhn-Tucker (KKT) conditions}~\cite{convexOptimization}, we have the following equations:
%The problem of ~\cite{prb-1} is a non-linear convex optimization problem, we using the Karush-Kuhn-Tucker (KKT) conditions to find the optimal value. More specifically, we have the following optimization problem:
% \begin{align}
% &\min_{\mathcal{M}} \sum_{i=1}^m \mathcal{M}_i ||\mathbf{r}_i||_0 \nonumber \\
% \label{prb-1-1}
% \text{subject to }  & KL(\mathbf{p}||\mathcal{M}) \leq \alpha. \\
% &M \in Simplex
% \end{align}
%Then, we apply KKT condition, we get the following result:
\begin{align}
%\label{prb-1-2}
\label{kkt1}
&\triangledown_{\mathcal{M}}(\sum_{i=1}^m \mathcal{M}_i^* ||\mathbf{r}_i||_0  + \mu_0 (KL(\mathbf{p}||\mathcal{M}^*) - \alpha) - \sum_{i=1}^m \mu_{i}\mathcal{M}_i^* \nonumber \\
& + \lambda (\sum_{i=1}^m \mathcal{M}_i^* -1))=\mathbf{0}  \\
%KL(\mathbf{p}||\mathcal{M}) - \alpha \leq 0 \nonumber \\
%\mu \geq 0 \nonumber \\
%u_{i} \geq 0, \forall i\in \{1,2,\cdots,m\} \nonumber \\
\label{kkt3}
&\mu_{i}\mathcal{M}_i^* = 0, \forall i\in \{1,2,\cdots,m\}  \\
\label{kkt4}
&\mu_0 (KL(\mathbf{p}||\mathcal{M}^*) - \alpha) =0,  
%\mathcal{M}_i > 0, \forall i\in \{1,2,\cdots,m\} \nonumber \\
%\sum_{i=1}^m \mathcal{M}_i = 1.
\end{align}
where $\triangledown$ indicates gradient, while $\mu_i$ and $\lambda$ are  called KKT multipliers.  
Then, we have the following equations:
\begin{align}
\label{e1}
&\mu_i = 0, \forall i\in \{1,2,\cdots,m\} \\
\label{e2}
&\mathcal{M}_{i}^*=\frac{\mu_0 {p}_{i}}{||\mathbf{r}_i||_0 + \lambda }, \forall i\in \{1,2,\cdots,m\}  \\
\label{e3}
&\mu_0=\frac{1}{\sum_{i=1}^m\frac{p_i}{||\mathbf{r}_i||_0 + \lambda}}  \\
\label{e4}
&KL(\mathbf{p}||\mathcal{M}^*) - \alpha = 0.
\end{align}
We briefly explain how we obtain Equations~\ref{e1}-\ref{e4} from the KKT conditions. First, according to Equation~\ref{kkt3} and $\mathcal{M}_i^*>0$, we have Equation~\ref{e1}. Then, according to Equation~\ref{kkt1} and Equation~\ref{e1}, we have Equation~\ref{e2}. Since $\sum_{i=1}^m \mathcal{M}_i^* = 1$, we further have Equation~\ref{e3}. Finally, we have Equation~\ref{e4} from Equation~\ref{kkt4} since $\mu_0\neq 0$.

By substituting $\mathcal{M}^*$ in Equation~\ref{e4} with Equation~\ref{e2} and Equation~\ref{e3}, we have a nonlinear equation with a single variable, i.e., $\lambda$. Then, we solve $\lambda$ in the equation using a standard iterative method in numerical analysis, e.g., we use the Newton's method in our experiments. After solving $\lambda$, we can obtain $\mu_0$ in Equation~\ref{e3} and then $\mathcal{M}_i^*$ in Equation~\ref{e2}.

%First, we using $\lambda$ to denote $\mu$, then, we can use $\lambda$ to denote $\mathcal{M}_{i}$, so now we can get a non-linear equation that only has one variable $\lambda$,  we can using iterative methods 
%to solve this equation. After we get the value of $\lambda$, we can get the value of $\mathcal{M}_{i}$.

\subsubsection{Scenario II: unknown $\mathbf{p}$ and known $C$}
We also follow the two-phase framework that we design for Scenario I. 
In Phase I, we use the same method in Algorithm~\ref{algorithm2} to find  the $m$ discrete noises $\{\mathbf{r}_1, \mathbf{r}_2, \cdots, \mathbf{r}_m\}$. 
However, in Phase II, we cannot use the method developed for Scenario I to find $\mathcal{M}^*$ because $\mathbf{p}$ is unknown.  
We observe that $KL(\mathbf{p}||\mathcal{M})\leq$ $\max_{\mathbf{p}} KL(\mathbf{p}||\mathcal{M})$ for any $\mathcal{M}$. 
Therefore, we address the challenge by relaxing the constraint $KL(\mathbf{p}||\mathcal{M})\leq \alpha$ as $\max_{\mathbf{p}} KL(\mathbf{p}||\mathcal{M})\leq \alpha$ in the optimization problem in Equation~\ref{prb-1}. Formally, we have: 
\begin{align}
%\textbf{Privacy-utility tradeoff } & \textbf{with a privacy-risk budget:} \nonumber \\
\mathcal{M}^*=&\argmin_{\mathcal{M}} \sum_{i=1}^m \mathcal{M}_i ||\mathbf{r}_i||_0 \nonumber \\
\label{prb-2}
\text{subject to }  & \max_{\mathbf{p}} KL(\mathbf{p}||\mathcal{M}) \leq \alpha \nonumber \\
& \mathcal{M}_i > 0, \forall i\in \{1,2,\cdots,m\} \nonumber \\
& \sum_{i=1}^m \mathcal{M}_i = 1,
\end{align}
%transforming Equation~\ref{prb-1} to the following relaxed optimization problem:
% \begin{align}
%%\textbf{Privacy-utility tradeoff } & \textbf{with a privacy-risk budget:} \nonumber \\
%&\min_{\mathcal{M}} \sum_{i=1}^m \mathcal{M}_i ||\mathbf{r}_i||_0 \nonumber \\
%\label{prb-2}
%\text{subject to }  & \max_{\mathbf{p}} KL(\mathbf{p}||\mathcal{M}) \leq \alpha.
%\end{align}
which means that the defender aims to preserve privacy within the budget for any prior probability distribution $\mathbf{p}$. 

Next, we discuss our \emph{analytical solution} for the above optimization problem. 
First, we can show that $\max_{\mathbf{p}} KL(\mathbf{p}||\mathcal{M}) = -\log (\mathcal{M}_{min})$, where $\mathcal{M}_{min}$ is the minimum one among $\{\mathcal{M}_{1}, $ $\mathcal{M}_{2}, \cdots, \mathcal{M}_{m} \}$. Therefore, we have $\mathcal{M}_{min} \geq e^{-\alpha}$. Suppose $||\mathbf{r}_{min}||_0$ is the smallest one among the $m$ noises. We note that $||\mathbf{r}_{min}||_0=0$ since PANDA does not add any noise for the attribute value that is originally inferred by the attacker's classifier. 
To minimize the utility loss, the defender adds the noise $\mathbf{r}_{i}$, whose $L_0$ norm is not the smallest, to the user's public data with the smallest non-zero probability $\mathcal{M}_{min}$; and the defender adds the noise $\mathbf{r}_{min}$ to the user's public data with the remaining probability. Formally, we have:
\begin{align}
\mathcal{M}_{i}^*=
\begin{cases}
\mathcal{M}_{min} & \text{ if } i \neq {min} \\
1- (m-1)\mathcal{M}_{min}   &\text{ otherwise},
\end{cases}
\end{align}
where $\mathcal{M}_{min}=\min \{e^{-\alpha},\frac{1}{m} \}$. Note that, when $e^{-\alpha} > \frac{1}{m}$, we let $\mathcal{M}_{min}=\frac{1}{m}$, which means that the defender selects one noise from  $\{\mathbf{r}_1, \mathbf{r}_2, \cdots, \mathbf{r}_m\}$ uniformly at random. 
%In the following, we have a discussion about how to solve above optimization problem, first, we simplify the constraints as follows:
%\begin{align}
%\max_{\mathbf{p}} KL(\mathbf{p}||\mathcal{M}) &\Leftrightarrow \\
%\max_{\mathbf{p}}(\sum_{i=1}^m \mathbf{p}_{i}\log (\mathbf{p}_{i})+\sum_{i=1}^m \mathbf{p}_{i}\log (\frac{1}{\mathcal{M}_i)}) &\Leftrightarrow \\
%\max_{\mathbf{p}}(\mathbf{p}_{min}\log (\mathcal{M}_min)) &\Leftrightarrow  \\
%\log (\frac{1}{\mathcal{M}_{min})})
%\end{align}
%Combined with other constraints, we have th following optimization problem:
% \begin{align}
%&\min_{\mathcal{M}} \sum_{i=1}^m \mathcal{M}_i ||\mathbf{r}_i||_0 \nonumber \\
%\text{subject to }&\log (\frac{1}{\mathcal{M}_{min})}) \leq \alpha \\
%&\mathcal{M}_{min} \leq \frac{1}{m}
%\end{align}
%The solution for this optimization are abvious. Because, when $\alpha < \log||m||$, there is no solutions, so we generalize the solution by sacrifice the privacy budget.
%First, we ranking the $||\mathbf{r}_i||_0$ descendingly.(If there are two number has the same value, we rank them randomly), after this, we have the following probability for $\mathcal{M}_{i}$. 
%\begin{align}
%\mathcal{M}_{i}&=\min \{e^{-\alpha},\frac{1}{m} \}, \forall i\in \{1,2,\cdots,m-1\} \\
%\mathcal{M}_{j}&=1- \sum_{i=1}^{m-1} \mathcal{M}_{i}, \forall j\in \{m\}
%\end{align}

\subsubsection{Scenario III and IV}
Again, we follow our two-phase framework to solve $\mathcal{M}$ for Scenario III and IV.  
Specifically, the defender learns a classifier $C_d$ to capture the relationship between a user's public data and attribute value. 
In reputation systems, the defender can collect rating scores and attribute values from users who disclose them publicly and learn the classifier $C_d$.   
When the public data are page likes on a social media, the defender can collect publicly available page likes and attribute values on the social media, to learn $C_d$. 
Then, the defender transforms the Scenario III (or IV) to Scenario I (or II) with the classifier $C$ replaced by $C_d$.  

Specifically, in Phase I, the defender finds the $m$ discrete noises $\{\mathbf{r}_1, \mathbf{r}_2, \cdots, \mathbf{r}_m\}$ to evade $C_d$, i.e., the defender uses our Algorithm~\ref{algorithm2} to solve the optimization problem in 
Equation~\ref{findr} with $C$ replaced by $C_d$. The discrete noise $\mathbf{r}_i$ is highly likely to also make the classifier $C$ predict attribute value $i$ for the user with noisy public data $\mathbf{x+r}_i$.  
This phenomena is called \emph{transferability} in adversarial machine learning~\cite{Goodfellow:ICLR:14b,nicolas2016transferability,liu2016delving}, i.e., an example optimized to evade one classifier is also highly likely to evade another classifier.
 Indeed, our experimental results in Section~\ref{exp} confirm such transferability.  In Phase II, the defender solves Equation~\ref{prb-1} and Equation~\ref{prb-2} to obtain  $\mathcal{M}^*$ for Scenario III and Scenario IV, respectively. 

%\neil{May show some theoretical analysis. Suppose $\mathcal{M}$ is obtained in Scenario I (or Scenario II) and $\mathcal{M}_d$ is obtained in Scenario III (or Scenario IV). First, when $C$ and $C_d$ have close accuracy, can we bound the difference between $\mathcal{M}$ and $\mathcal{M}_d$, as well as difference between $KL(\mathbf{p}||\mathcal{M})$ (or $\max_{\mathbf{p}} KL(\mathbf{p}||\mathcal{M})$) and $KL(\mathbf{p}||\mathcal{M}_d)$ (or $\max_{\mathbf{p}} KL(\mathbf{p}||\mathcal{M}_d)$). }


\subsection{Inference-Attack Defense Problem II}
Similar to solving the Inference-Attack Defense Problem I, we consider the four scenarios and follow our two-phase framework.
In Phase I,  to find the $m$ discrete noises  $\{\mathbf{r}_1, \mathbf{r}_2, \cdots, \mathbf{r}_m\}$, we solve Equation~\ref{findr} for Scenario I and Scenario II, while we solve  Equation~\ref{findr} with the classifier $C$ replaced by $C_d$ for Scenario III and Scenario IV. Next, we discuss more details about Phase II to find $\mathcal{M}^{**}$. 

\myparatight{Finding $\mathcal{M}^{**}$ for Scenario I and III} Again, in our framework, $\mathcal{M}^{**}$ is a probability distribution over the $m$ noises, i.e., the defender adds the noise $\mathbf{r}_i$ to $\mathbf{x}$ with a probability $\mathcal{M}_i^{**}$. Then, we can transform Equation~\ref{ulb} to the following optimization problem: 
\begin{align}
%\textbf{Privacy-utility tradeoff } & \textbf{with a privacy-risk budget:} \nonumber \\
\mathcal{M}^{**}=&\argmin_{\mathcal{M}} KL(\mathbf{p}||\mathcal{M}) \nonumber \\
\label{ulb-1}
\text{subject to }  & \sum_{i=1}^m \mathcal{M}_i ||\mathbf{r}_i||_0 \leq \beta \nonumber \\
& \mathcal{M}_i > 0, \forall i\in \{1,2,\cdots,m\} \nonumber \\
& \sum_{i=1}^m \mathcal{M}_i = 1.
\end{align}

We can show that the above optimization problem is convex. Moreover, according to the KKT conditions, we have:
%In the next, we discuss how to solve the following optimization problem:
% \begin{align}
% &\min_{\mathcal{M}} KL(\mathbf{p}||\mathcal{M}) \nonumber \\
% \text{subject to }  & \sum_{i=1}^m \mathcal{M}_i ||\mathbf{r}_i||_0 \leq \beta \\
% & \mathcal{M}_i > 0, \forall i\in \{1,2,\cdots,m\} \nonumber \\
% & \sum_{i=1}^m \mathcal{M}_i = 1.
% \end{align}
%Then, we apply KKT condition, we get the following result:
\begin{align}
&\triangledown_{\mathcal{M}}(KL(\mathbf{p}||\mathcal{M}^{**}) + \mu_0 (\sum_{i=1}^m \mathcal{M}_i^{**} ||\mathbf{r}_i||_0 - \beta) - \sum_{i=1}^m \mu_{i}\mathcal{M}_i^{**} \nonumber \\
& + \lambda (\sum_{i=1}^m \mathcal{M}_i^{**} -1))=0  \\
%\sum_{i=1}^m \mathcal{M}_i ||\mathbf{r}_i||_0 - \beta \leq 0 \nonumber \\
%\mu \geq 0 \nonumber \\
%u_{i} \geq 0, \forall i\in \{1,2,\cdots,m\} \nonumber \\
&\mu_{i}\mathcal{M}_i^{**} = 0, \forall i\in \{1,2,\cdots,m\}  \\
&\mu_0 (\sum_{i=1}^m \mathcal{M}_i^{**} ||\mathbf{r}_i||_0 - \beta) =0.
%\mathcal{M}_i > 0, \forall i\in \{1,2,\cdots,m\} \nonumber \\
%\sum_{i=1}^m \mathcal{M}_i = 1.
\end{align}

Then, we can obtain the following equations:
\begin{align}
\label{prb-1-3}
&\mu_i = 0, \forall i\in \{1,2,\cdots,m\} \\
\label{ex1}
&\mathcal{M}_{i}^{**}=\frac{{p}_{i}}{\mu_0 ||\mathbf{r}_i||_0 + \lambda } \\
\label{ex2}
&\sum_{i=1}^m \mathcal{M}_i^{**} ||\mathbf{r}_i||_0 - \beta = 0 \\
\label{ex3}
&\mu_0=\frac{1-\lambda}{\beta}.
\end{align}
Via substituting $\mathcal{M}_{i}^{**}$ in Equation~\ref{ex2} with Equation~\ref{ex1} and Equation~\ref{ex3}, we obtain a nonlinear equation with a single variable $\lambda$. We use the Newton's method to solve $\lambda$, and then we can obtain $\mu_0$ in Equation~\ref{ex3} and $\mathcal{M}^{**}$ from Equation~\ref{ex1}.


\myparatight{Finding $\mathcal{M}^{**}$ for Scenario II and IV} In these two scenarios, the prior probability distribution $\mathbf{p}$ is unknown to the defender. Since $\max_{\mathbf{p}} KL(\mathbf{p}||\mathcal{M})$ is an upper bound of the privacy risk $KL(\mathbf{p}||\mathcal{M})$, we propose to minimize the upper bound while satisfying the utility loss. Formally, we relax the optimization problem in Equation~\ref{ulb-1} as follows: 
\begin{align}
%\textbf{Privacy-utility tradeoff } & \textbf{with a privacy-risk budget:} \nonumber \\
\mathcal{M}^{**}=&\argmin_{\mathcal{M}} \max_{\mathbf{p}} KL(\mathbf{p}||\mathcal{M}) \nonumber \\
\label{ulb-2}
\text{subject to }  & \sum_{i=1}^m \mathcal{M}_i ||\mathbf{r}_i||_0 \leq \beta \nonumber \\
&\mathcal{M}_i > 0, \forall i\in \{1,2,\cdots,m\} \nonumber \\
&\sum_{i=1}^m \mathcal{M}_i = 1.
\end{align}

Next, we derive an analytical solution for the above optimization problem. 
Since $\max_{\mathbf{p}} KL(\mathbf{p}||\mathcal{M}) = -\log (\mathcal{M}_{min})$, the objective function $\argmin_{\mathcal{M}} \max_{\mathbf{p}} KL(\mathbf{p}||\mathcal{M})$ is equivalent to $\argmax_{\mathcal{M}} \mathcal{M}_{min}$. We also have $\mathcal{M}_{min} \sum_{i \neq min} ||\mathbf{r}_i||_0 + (1- (m-1)\mathcal{M}_{min}) ||\mathbf{r}_{min}||_0$ $\leq$ $\sum_{i=1}^m \mathcal{M}_i ||\mathbf{r}_i||_0$ $\leq \beta$, where $\mathbf{r}_{min}$ is the noise with the smallest $L_0$ norm. Therefore, we have $\mathcal{M}_{min}$ $\leq$ $\frac{\beta-||\mathbf{r}_{min}||_0}{\sum_{i \neq min} ||\mathbf{r}_i||_0 - (m-1)||\mathbf{r}_{min}||_0}$. Furthermore, we have $\mathcal{M}_{min} \leq \frac{1}{m}$. 
Thus, we have the following solution:
\begin{align}
\mathcal{M}_{i}^{**}=
\begin{cases}
\mathcal{M}_{min} & \text{ if } i \neq {min} \\
1- (m-1)\mathcal{M}_{min}   &\text{ otherwise},
\end{cases}
\end{align}
where $\mathcal{M}_{min}=\min \{\frac{\beta-||\mathbf{r}_{min}||_0}{\sum_{i \neq min} ||\mathbf{r}_i||_0 - (m-1)||\mathbf{r}_{min}||_0},\frac{1}{m}\}$. 

%Like above, we will first simplify the optimization function first.
%\begin{align}
%\max_{\mathbf{p}} KL(\mathbf{p}||\mathcal{M}) \Leftrightarrow \log(\frac{1}{\mathcal{M}_{min}})
%\end{align}
%Thus, we got the following optimization problem:
%\begin{align}
%&\min_{\mathcal{M}} \log(\frac{1}{\mathcal{M}_{min}}) \\
%\text{subject to }  & \sum_{i=1}^m \mathcal{M}_i ||\mathbf{r}_i||_0 \leq \beta \nonumber \\
%&\mathcal{M}_i > 0, \forall i\in \{1,2,\cdots,m\} \nonumber \\
%&\sum_{i=1}^m \mathcal{M}_i = 1.
%\end{align}
%Thus, we have the following convex optimization problem.
%\begin{align}
%&\max_{\mathcal{M}} \mathcal{M}_{min} \\
%\text{subject to }  & \sum_{i=1}^m \mathcal{M}_i ||\mathbf{r}_i||_0 \leq \beta \\
%&\mathcal{M}_i > 0, \forall i\in \{1,2,\cdots,m\} \nonumber \\
%&\sum_{i=1}^m \mathcal{M}_i = 1.
%\end{align}
%First, we ranking the $||\mathbf{r}_i||_0$ descendingly.(If there are two number has the same value, we rank them randomly), after this, we have the following probability for $\mathcal{M}_{i}$. 
%\begin{align}
%\mathcal{M}_{i}&=\min \{\frac{\beta}{\sum_{i=1}^m ||\mathbf{r}_i||_0},\frac{1}{m} \}, \forall i\in \{1,2,\cdots,m-1\} \nonumber \\
%\mathcal{M}_{j}&=1- \sum_{i=1}^{m-1} \mathcal{M}_{i}, \forall j \in \{m\}
%\end{align}

%\begin{algorithm}[t]
%\caption{Noise }
%\label{algorithm2}
%\begin{algorithmic}
%\REQUIRE Public data $\textbf{x}$, classifier $\textbf{C}$, noise-type-policy $\mathcal{P}$ and target attribute value $i$. \\
%\ENSURE  Noise $\textbf{r}_i$. \\
%    %Initialize $\textbf{x}_{0}=\textbf{x}$ \\
%    Initialize $t=0,\overline{\textbf{x}}=\textbf{x}$. \;
%%\noindent \textbf{Process:}
%%\PROCESS ~~\\
%    %\WHILE { $\sum_{u\in V}|\hat{{p}}_u^{(t)} - \hat{{p}}_u^{(t-1)}| \geq \delta$ and $t \leq T$} \;
%	%\IF{$\textbf{C}(\textbf{x})==i$} \RETURN $\textbf{0}$ \ENDIF \\
%	
%	\WHILE { $\textbf{C}(\overline{\textbf{x}}) \neq i$ and $t \leq \text{maxiter}$} \;
%	\STATE //Find the entry to be modified. \;
%	\IF{$\mathcal{P}==Add\_New$} \;
%	
%	\STATE $e_{inc}=\argmax_{j} \{\frac{\partial \textbf{C}_{i}(\overline{\mathbf{x}})}{\partial \mathbf{x}_j}| \mathbf{x}_j=0\} $ \;
%	\ENDIF\;
%	
%	\IF{$\mathcal{P}==Modify\_Exist$} \;
%	\STATE $e_{inc}=\argmax_{j} \{(1-\overline{\textbf{x}}_j) \frac{\partial \textbf{C}_{i}(\overline{\mathbf{x}})}{\partial \mathbf{x}_j}| \mathbf{x}_j \neq 0\}$ \;
%	
%	%(\textbf{1}-\overline{\textbf{x}})\times \triangledown \textbf{C}_{i}$ \\
%	\STATE $e_{dec}=\argmax_{j} \overline{\textbf{x}} \times (\textbf{-1}) \times \triangledown \textbf{C}_{i}$ \\
%	\ENDIF \\
%
%
%	\IF{$\mathcal{P}==Modify\_Add$} \;
%	\STATE $i_{inc}=\argmax_{j} (\textbf{1}-\overline{\textbf{x}})\times \triangledown \textbf{C}_{i}$ \\
%	\STATE $value\_inc=(\textbf{1}-\overline{\textbf{x}}) \times \textbf{C}_{i}[i_{inc}]$ \\
%	\STATE $i_{dec}=\argmax_{j} \overline{\textbf{x}} \times (\textbf{-1}) \times \triangledown \textbf{C}_{i}$ \\
%	\STATE $value\_dec=(\overline{\textbf{x}} \times (\textbf{-1}) \times \triangledown \textbf{C}_{i})[i_{dec}]$ \\
%	\ENDIF \\
%
%
%	%\triangledown \textbf{C}_{i}$ \\
%%	\WHILE { $\triangledown \textbf{C}_{i}(i_{inc}) > 0 $ and $\overline{\textbf{x}}(i_{inc})<1$} \;
%%	\STATE $\overline{\textbf{x}}+=\tau$ \\	
%%	\ENDWHILE \\
%%	
%%	\ELSE \;
%%	
%%	\IF{$\mathcal{P}==Modify\_Add$} \;
%%	\STATE $i_{inc}=\argmax_{j} (\textbf{1}-\overline{\textbf{x}})\times \triangledown \textbf{C}_{i}$ \\
%%	\STATE $value\_inc=(\textbf{1}-\overline{\textbf{x}}) \times \textbf{C}_{i}[i_{inc}]$ \\
%%	\STATE $i_{dec}=\argmax_{j} \overline{\textbf{x}} \times (\textbf{-1}) \times \triangledown \textbf{C}_{i}$ \\
%%	\STATE $value\_dec=(\overline{\textbf{x}} \times (\textbf{-1}) \times \triangledown \textbf{C}_{i})[i_{dec}]$ \\
%%	\ENDIF \\
%%	
%%	\IF{$\mathcal{P}==Modify\_Existing$} \;
%%	\STATE $i_{inc}=\argmax_{j|x_{0}(j)\neq 0} (\textbf{1}-\overline{\textbf{x}})\times \triangledown \textbf{C}_{i}$ \\
%%	\STATE $value\_inc=(\textbf{1}-\overline{\textbf{x}}) \times \textbf{C}_{i}[i_{inc}]$ \\
%%	\STATE $i_{dec}=\argmax_{j|x_{0}(j)\neq 0} \overline{\textbf{x}} \times (\textbf{-1}) \times \triangledown \textbf{C}_{i}$ \\
%%	\STATE $value\_dec=(\overline{\textbf{x}} \times (\textbf{-1}) \times \triangledown \textbf{C}_{i})[i_{dec}]$ \\
%%	\ENDIF \\
%%	
%%	\IF {$value\_inc \geq  value\_dec$} \;
%%	\WHILE { $\triangledown \textbf{C}_{i}(i_{inc}) > 0 $ and $\overline{\textbf{x}}(i_{inc})<1$} \;
%%	\STATE $\overline{\textbf{x}}[i_{inc}]+=\tau$ \\
%%	\ENDWHILE \\
%%	\ELSE \;
%%	\WHILE { $\triangledown \textbf{C}_{i}(i_{dec}) < 0 $ and $\overline{\textbf{x}}(i_{dec})>0$} \;
%%	\STATE $\overline{\textbf{x}}[i_{dec}]-=\tau$ \\
%%	\ENDWHILE \\
%%	\ENDIF \\
%%	\ENDIF \\
%%	\STATE $t=t+1$ \\
%	\ENDWHILE \\
%%	
%	\RETURN $\overline{\textbf{x}}-\textbf{x}$. \\
%
%    % \WHILE { $\textbf{F}(\textbf{x}_{i}) \neq l_{t}$ and $i \leq maxiter$} \;
%	% \STATE $i_{max1}=\argmax_{j} (\textbf{1}-\textbf{x}_{i})\times \triangledown \textbf{F}_{l_{t}}$ \\
%	% \STATE $value=(\textbf{1}-\textbf{x}_{i}) \times \textbf{F}_{l_{t}}[i_{max1}]$ \\	
%	% \STATE $i_{decrease}=\argmax_{j} \textbf{x}_{i} \times (\textbf{-1}) \times \triangledown \textbf{F}_{l_{t}}$ \\
%	% \IF {$value \geq  \textbf{x}_{i} \times (-\textbf{1})\times \triangledown \textbf{F}_{l_{t}}[i_{decrease}]$} \;
%	% %\STATE $i_{max}=i_{max1}$ \\
%	% \STATE $\textbf{r}_{i}[i_{max1}]$=1.0 \\
%	% \ELSE \;
%	% %\STATE $i_{max}=i_{max2}$ \\
%	% \STATE $\textbf{r}_{i}[i_{max2}]$=0.0 \\
%	% \ENDIF \\
%	% \STATE $\textbf{x}_{i+1}=\textbf{x}_{i}+\textbf{r}_{i}$ \\
%	% \STATE $i=i+1$ \\
%    % \ENDWHILE \\
%    % \RETURN $\widehat{\textbf{r}}=\sum_{i}\textbf{r}_{i}$. \\
%\end{algorithmic}
%\end{algorithm}


%\subsection{Notation}
%The user $i$ is denoted as $u_{i}$. And for each user, it would rating some apps, we denoted the origin apps the user rated as $x_{i}$, in 
%order to protect user's privacy, we would add some noise to $x_{i}$, which is denoted as $x_{n}$ which can be seen as a random variable has some ditribution, denoted as $P(x_{n})$. Those two are a vector whose index 
%denoted the number of app and the value denoted the app rating score. We using $C$ to denote the city. The distribution of city $C$ is 
%denoted as $P_{C}$. And we have the following defintion:
%
%\subsection{Basic Definition}
%\begin{definition}
%(Distance) Two app rating instance, named $x_{i}$, $x_{n}$ distance is: $d_{u}(x_{i},x_{n})=abs(x_{i}-x_{n})$
%\end{definition}
%
%\begin{definition}
%(User's City Classifier Conditional distribution)  For a user $u$'s $x_{n}$ certain distribution and corresponds classifier $\mathbf{F}$, this user's city's conditional distribution is 
%defined as:
%\begin{eqnarray}
%P_{\mathbf{F}|x_{n}}(C=c)=P(c=\mathbf{F}(x_{n}))
%\end{eqnarray}
%\end{definition}
%
%\begin{definition}
%$\epsilon$-KL-Privacy. For user $u$, a mechanism $P_{\mathbf{F}|x_{n}}$ satisfies $\epsilon$-KL-Privacy if 
%there exists distribution of $x_{n}$, $s.t.$
%\begin{eqnarray}
%\mathbf{D}(P_{\mathbf{F}|x_{n}}|P_{C})\leq \epsilon
%\end{eqnarray}
%\end{definition}
%
%\begin{definition}
%KL-IL. For user $u$, a mechanism $P_{\mathbf{F}|x_{n}}$'s KL-IL is 
%defined as:
%\begin{eqnarray}
%\mathbf{D}(P_{\mathbf{F}|x_{n}}|P_{C})
%\end{eqnarray}
%\end{definition}
%
%\subsection{Optimization Problem}
%\subsubsection{Known Prior}
%First, we assume an attacker user's certain mechanism to infer user's private information.
%In order to add minimal noise to protect user's privacy, that is, satisfies $\epsilon$-KL-Privacy, we have the following optimization problem.
%\begin{definition}
%(Optimization Problem)  For a user $u$'s $x_{n}$ and certain mechanism $P_{\mathbf{F}|x_{n}}$, to find a certain distribution $P(x_{n})$ to satifies $\epsilon$-KL-Privacy is to solve the following optimization problem.
%\begin{eqnarray}
%\min_{P(x_{n})}E(d_{u}(x_{0},x_{n}))
%\end{eqnarray}
%s.t.
%\begin{eqnarray}
%\mathbf{D}(P_{\mathbf{F}|x_{n}}|P_{C})\leq \epsilon
%\end{eqnarray}
%\end{definition}
%
%To solve the above optimization problem is non-trival. In the following, we will describe our algorithm to solve the above problem.
%First, we start by describing an algorithm template or meta-algorithm. The inputs are a user's($u$) original rated app($x_{0}$), a mechanism $P_{\mathbf{F}|x_{n}}$ 
%and attacker's prior probability regarding city $P_{C}$.
%
%The three main components of our algorithm are the $\mathbf{MiniNoise}$, $\mathbf{CompuProb}$ and $\mathbf{AddNoise}$.
%
%The $\mathbf{MiniNoise}$ is to solve the following optimization problem for each city. The result is a vector $\mathbf{r}$ whose index is the number of the city 
%and the value is $d_{u}(x_{0}-x_{n})$ where $x_{n}$ is the solution  of the following optimization problem regarding city $l_{t}$.
%\begin{lemma}
%\begin{eqnarray}
%\min_{x_{n}}d_{u}(x_{0},x_{n})
%\end{eqnarray}
%s.t.
%\begin{eqnarray}
%\mathbf{F}(x_{n})=l_{t}
%\end{eqnarray}
%\end{lemma}
%
%The $\mathbf{CompuProb}$ is to find the one of the probability distrbution $P_{x_{n}}$ makes it satisfies the above optimization. Because for each city, we have 
%find an instance of $x_{n}$ which makes $F(x_{n})=l_{t}$. Thus, we can assign each them of a probability and then solve the following optimization problem to find the 
%exact probability. This probability distrbution is one of the solution of our optimization problem.
%\begin{lemma}
%\begin{eqnarray}
%\min_{P_{x_{n}}}\mathbf{P_{x_{n}}r}
%\end{eqnarray}
%s.t.
%\begin{eqnarray}
%\mathbf{D}(P_{\mathbf{F}|x_{n}}|P_{C})\leq \epsilon
%\end{eqnarray}
%\end{lemma}
%
%The $\mathbf{AddNoise}$ is to add noise according to the probability of $x_{n}$, i.e. $P_{x_{n}}$.
%However, sometimes a user may don't want add much noise and think sacrifice a little bit privacy leakage is acceptable. 
%In this situation, we will have the following opmization.
%
%To be done.
%
%\begin{definition}
%(Optimization Problem)  For a user $u$'s $x_{n}$ and certain mechanism $P_{\mathbf{F}|x_{n}}$, to find a certain distribution $P(x_{n})$ to satifies ($\varepsilon ,\delta$)-Privacy is to solve the following optimization problem.
%\begin{eqnarray}
%\min_{P(x_{n})}\mathbf{D}(P_{\mathbf{F}|x_{n}}|P_{C})
%\end{eqnarray}
%s.t.
%\begin{eqnarray}
%E(d_{u}(x_{0},x_{n}))\leq \varepsilon
%\end{eqnarray}
%\end{definition}
%\subsubsection{Unknow Prior}
%If the attacker don't know the prior, then, we have the following optimization problem.
%\begin{definition}
%(Optimization Problem)  For a user $u$'s $x_{n}$ and certain mechanism $P_{\mathbf{F}|x_{n}}$, to find a certain distribution $P(x_{n})$ to satifies $\epsilon$-KL-Privacy is to solve the following optimization problem.
%\begin{eqnarray}
%\min_{P(x_{n})}E(d_{u}(x_{0},x_{n}))
%\end{eqnarray}
%s.t.
%\begin{eqnarray}
%\max_{P_{C}}\mathbf{D}(P_{\mathbf{F}|x_{n}}|P_{C})\leq \epsilon
%\end{eqnarray}
%\end{definition}
%Similarly, if user don't want to add that much noise can satisfies some privacy leakage, we have the following optimization problem.
%\begin{definition}
%(Optimization Problem)  For a user $u$'s $x_{n}$ and certain mechanism $P_{\mathbf{F}|x_{n}}$, to find a certain distribution $P(x_{n})$ to satifies ($\varepsilon ,\delta$)-Privacy is to solve the following optimization problem.
%\begin{eqnarray}
%\min_{P(x_{n})}\max_{P(C)}\mathbf{D}(P_{\mathbf{F}|x_{n}}|P_{C})
%\end{eqnarray}
%s.t.
%\begin{eqnarray}
%E(d_{u}(x_{0},x_{n}))\leq \varepsilon
%\end{eqnarray}
%\end{definition}

==> model.tex <==
\section{Design of AttriInfer}
\subsection{Overview}
Suppose we consider a binary attribute $A$. 
Given a training dataset, we first use user behaviors to learn a binary classifier for the attribute. 
Then, we use the classifier to predict the probability that each target user has the attribute $A$. 
We call this probability \emph{prior probability}. 
We use a binary random variable to model each user, and we model the joint probability distribution of all binary random variables as a pairwise Markov Random Field (pMRF) based on the structure of the social network. 
Given the training dataset and prior probability, we propagate label information among the social graph via the pMRF model. After the propagation, we obtain a posterior probability of having the attribute for each target user. Then, we use the posterior probability to predict whether a target user has the attribute or not. In this section, we introduce a basic version of AttriInfer, in which we use Loopy Belief Propagation (LBP) to infer the posterior probabilities. 



\subsection{Learning Prior using Behaviors}
We associate a binary random variable $x_u$ with each user $u$, where $x_u=1$ means that $u$ has the attribute $A$ and $x_u=-1$ means that $u$ does not have the attribute. %$\bar{x}_u$ indicates the observed value 
We denote the behaviors of a user $u$ as a \emph{behavior vector} $\vec{b}_u$. The vector $\vec{b}_u$ can be a binary vector, where an entry is 1 if and only if $u$ has performed a certain action on the corresponding object. For instance, when we consider page likes as behaviors, an entry of 1 means that the user liked the corresponding page. The behavior vector $\vec{b}_u$ can also be a real-valued vector. For instance, when we consider reviews as behaviors, an entry is the rating score that a user gave to the corresponding item (e.g., app, movie, book). Likewise, when we consider {clickstream} as behaviors, an entry of a user's behavior vector can be the frequency of a certain subsequence (consisting of click events and discretized time gaps between them) that appears in the user's clickstream~\cite{Wang13Clickstream,WangCHI16}. 


We learn the prior probability of target users using a standard {logistic regression classifier}.
Specifically,  the probability $q_u$ that  $u$ has the attribute $A$ is modeled as $q_u=Pr(x_u=1)=\frac{1}{1 + exp(-h_u)}$, where $h_u=\vec{b}_u ^T\cdot \vec{c} + d$.  $d$ and the vector $\vec{c}$ are parameters of the logistic regression classifier. 
Given a training dataset, in which each user has behaviors,  we can learn these parameters via \emph{maximum likelihood estimation}. In our experiments, we leverage the library LIBLINEAR~\cite{liblinear08} to learn these parameters.  We note that we choose logistic regression classifier instead of a Support Vector Machine (SVM) because SVM does not directly produce a probability that a user has the attribute.\footnote{We note that SVM's outputs can be transformed into probabilities~\cite{liblinear08}, but they achieve suboptimal performance.} With this logistic regression classifier, we can compute the prior probability for each user who has behaviors. 
A user has a prior probability of 0.5 if it does not have behaviors.
%  has a prior probability of 0.5. %For a training user who has the attribute, we set its prior probability to be close to 1 (e.g., 0.9 in our experiments)
%For a users in the training dataset, we set 

\subsection{Propagating Prior Using Social Graph}
 We leverage a pMRF to model the social graph, with which we can propagate the prior probability among the social graph to compute a posterior probability that each target user has the attribute. 
\subsubsection{Intuitions} 
We  denote by $\Gamma_u$ the set of  $u$'s neighbors in the social network, and $\bar{x}_{\Gamma_u}$ the observed states (whether having the attribute or not) of the neighbors. 
Social networks are known to have the \emph{homophily} property~\cite{homopily01}, i.e., if we sample an edge $(u,v)$ from a social graph uniformly at random, the two users $u$ and $v$ are highly likely to both have the attribute or both not have the attribute. Based on this homophily intuition, we model the probability that a user $u$ has the attribute $A$ 
when the user's neighbors' states are already known  
as follows:
\begin{align}
\label{local_rule}
Pr(x_u=1|\bar{x}_{\Gamma_u})=\frac{1}{1+\text{exp}(-\sum_{v\in \Gamma_u}J_{uv}\bar{x}_v - h_u)} \ ,
\end{align}
where $J_{uv} > 0$ is the homophily strength between $u$ and $v$, and $h_u$ characterizes $u$'s  prior knowledge obtained through the logistic regression classifier.  A higher $J_{uv} $ means that $u$ and $v$ are more likely to have the same state. 


%Specifically, $J_{uv}>0$ means $u$ and $v$ tend to have the same state;  $J_{uv}<0$ indicates $u$ and $v$ tend to have opposite states; and $J_{uv}=0$ indicates that there is no coupling between them. In practice, these coupling strengths can encode trust levels between nodes. 
%%In these variables we encode our general homophily assumption, i.e. we set them to a global (independent from $u$,$v$) positive value.
%
%Note that our local rule in Equation~\ref{local_rule} incorporates the homophily assumption via setting $J_{uv}>0$.
%
 

\subsubsection{A Pairwise Markov Random Field}
We find that Equation~\ref{local_rule} can be achieved by modeling the social graph as a pairwise Markov Random Field (pMRF). A pMRF defines a joint probability distribution for binary random variables associated with all the users in the social graph. Generally speaking, a pMRF is specified by a \emph{node potential} for each user $u$, which incorporates prior probability about $u$, and an \emph{edge potential} for each edge $(u,v)$, which represents correlations between $x_u$ and $x_v$.  In our attribute inference problem, we define a node potential $\phi_u(x_u)$ for user $u$ as
\begin{displaymath}
\phi_u(x_u):=
\begin{cases} 
q_u  & \text{if } x_u = 1  \\ 
1-q_u  &  \text{if } x_u = -1
\end{cases} 
\end{displaymath}
and an \emph{edge potential  $\varphi_{uv}(x_u, x_v)$} for the edge $(u,v)$ as
\begin{displaymath}
\varphi_{uv}(x_u, x_v):=
\begin{cases} 
w_{uv} & \text{if } x_u x_v = 1  \\  
1 - w_{uv} &  \text{if } x_u x_v = -1 \ ,
\end{cases}
\end{displaymath}
where $w_{uv}\!:=\!(\!1+\!\mathrm{exp}\{-J_{uv}\})^{-1}$. 
Then, the following pMRF satisfies Equation~\ref{local_rule} for every user.
$$Pr(x_V)= \frac{1}{Z}\prod_{u\in V} \phi_u(x_u) \prod_{(u, v)\in E} \varphi_{uv}(x_u, x_v)\ ,$$
where $Z=\sum_{x_u}\prod_{u\in V} \phi_u(x_u) \prod_{(u, v)\in E} \varphi_{uv}(x_u, x_v)$ is called the partition function and normalizes the probabilities.
%The  edge potential $\varphi_{uv}(x_u, x_v)$ encodes the homophily strength of two linked users $u$ and $v$. The larger $w_{uv}$ is, the stronger the model favors $u$ and $v$ to have the same state.   More precisely,  $w_{uv} > 0.5$ means connected nodes tend to have the same state; $w_{uv} < 0.5$ means connected nodes tend to have opposite states; $w_{uv}=0.5$ encodes the scenario where there is no coupling between $u$ and $v$.  Note that setting $w_{uv} > 0.5$ encodes our homophily assumption.
$w_{uv} > 0.5$ captures the homophily property.  
In our definitions, $w_{uv}$ can be interpreted as the probability that two linked users  have the same state. In this work, we set $w_{uv}=w>0.5$ for all edges, and we call $w$ \emph{homophily strength}.  
However, learning the parameters $w_{uv}$ for different edges would be a valuable future work. 

\subsubsection{Estimating Posterior Probability using LBP}
We compute the \emph{posterior probability distribution} of a user $u$, i.e., 
$Pr(x_u) = \sum_{x_{V/u}} Pr(x_V)$. For simplicity, we denote by $p_u$ the posterior probability that 
$u$ has the attribute, i.e., $p_u=Pr(x_u=1)$.  
 This posterior probability is used to predict whether a user has the attribute or not.  
In the basic version of AttriInfer, we use Loopy Belief Propagation (LBP)~\cite{Pearl88} to estimate the posterior probability distribution $Pr(x_u)$. 
LBP iteratively passes messages between neighboring users in the graph. Specifically, the message $m_{vu}^{(t)}(x_u)$ sent from $v$ to $u$ in the $t$th iteration is 
\begin{align}
\label{message}
m_{vu}^{(t)}(x_u) = \sum_{x_v} \phi_v (x_v) \varphi_{vu}(x_v, x_u) \prod_{k \in \Gamma(v)/u} m_{kv}^{(t-1)}(x_v),
\end{align} 
where $\Gamma(v)/u$ is the set of all neighbors of $v$, except the receiver node $u$. This encodes that each node %essentially
 forwards a product over  incoming messages of the last iteration and adapts this message to the respective receiver based on the homophily strength with the receiver. LBP stops when the changes of messages  become negligible in two consecutive iterations (e.g., $l_1$ distance of changes becomes smaller than $10^{-3}$) or it reaches the predefined maximum number of iterations $T$. After LBP halts, we estimate the posterior probability distribution $Pr(x_u)$ as follows:
 \begin{align}
 \small
 \label{posteriorfull}
 Pr^{(t)}(x_u)\propto \phi_u (x_u) \prod_{k \in \Gamma(u)} m_{ku}^{(t)}(x_u),
 \end{align} 
which is equivalent to
\begin{align}
 \label{belief}
 \begin{split}
 & p_u^{(t)}=\frac{q_u \prod\limits_{k \in \Gamma(u)} m_{ku}^{(t)}}{q_u \prod\limits_{k \in \Gamma(u)} m_{ku}^{(t)} + (1-q_u) \prod\limits_{k \in \Gamma(u)} (1-m_{ku}^{(t)})}, \\
 \end{split}
 \end{align} 
 where $m_{ku}^{(t)}=m_{ku}^{(t)}(x_u=1)$ and $1-m_{ku}^{(t)}=m_{ku}^{(t)}(x_u=-1)$.
 Note that normalizing $m_{ku}^{(t)}(x_u)$ does not affect the computation of posterior probability distribution of any user. 
 Therefore, for simplicity, we have normalized  $m_{ku}^{(t)}(x_u)$ such that  $m_{ku}^{(t)}(x_u=1)$ + $m_{ku}^{(t)}(x_u=-1)=1$ in the above equation. 

We note that pMRF and LBP were also adopted to detect Sybils in OSNs~\cite{sybilbelief}. 
Sybil detection and attribute inference for binary attributes are algorithmically similar. 
However, previous work~\cite{sybilbelief} didn't perform optimization and convergence analysis as we will discuss 
in the next two sections Section~\ref{optimization} and Section~\ref{sec:cvgAnal}.  

\section{Optimizing AttriInfer}
\label{optimization}
The basic version of AttriInfer has two shortcomings: 
1) AttriInfer is not scalable enough, and 2) AttriInfer is an iterative method but is not guaranteed to converge. 
Being not convergent makes it hard to select an appropriate number of iterations. 
The reason is that LBP maintains messages on each edge and  LBP might oscillate on loopy graphs~\cite{Pearl88}.
Therefore, we further optimize AttriInfer to address these shortcomings. 

\subsection{Eliminating Message Maintenance}
One of the major reasons why basic AttriInfer is not scalable enough is that LBP maintains messages on each edge. 
We observe that the key reason why LBP needs to maintain messages on edges is that  when  a node $v$ prepares a message to its neighbor $u$, it excludes the message that $u$ sent to $v$.  
Therefore, our first optimization step is to include the message that $u$ sent to $v$ when $v$ prepares its message for $u$. 
Formally, we approximate Equation~\ref{message} as:
\begin{align}
%\label{message}
m_{vu}^{(t)}(x_u) = \sum_{x_v} \phi_v (x_v) \varphi_{vu}(x_v, x_u) \prod_{k \in \Gamma(v)} m_{kv}^{(t-1)}(x_v).
\end{align} 

Considering Equation~\ref{posteriorfull}, we have:
\begin{align}
m_{vu}^{(t)}(x_u) \propto \sum_{x_v} \varphi_{vu}(x_v, x_u) Pr^{(t-1)}(x_v).
\end{align}
Recall that we normalize  $m_{vu}^{(t)}(x_u)$ such that  $m_{vu}^{(t)}(x_u=1)$ + $m_{vu}^{(t)}(x_u=-1)=1$, and we abbreviate $m_{vu}^{(t)}(x_u=1)$ as $m_{vu}^{(t)}$.  With such normalization,  our new messages become:
\begin{equation}
\small
\label{modifiedMessage}
m_{vu}^{(t)} = p_v^{(t-1)} w + (1-p_v^{(t-1)})(1-w).
\end{equation}
AttriInfer does not need to maintain messages on edges using our new messages. 

\subsection{Linearizing as a Matrix Form} 
AttriInfer iteratively applies Equations~\ref{modifiedMessage} and~\ref{belief} using our new messages,
which still cannot guarantee convergence. 
The key reason is that Equation~\ref{belief} combines messages from a user's neighbors \emph{nonlinearly}. 
We make AttriInfer converge via linearizing Equation~\ref{belief}. 
The resulting optimized AttriInfer can be represented in a concise matrix form. 
Before introducing our linearization, we define some terms. 
In particular, we define the \emph{residual} $\hat{y}$ of a variable $y$ as $\hat{y}=y-0.5$; 
and we define the \emph{residual vector} $\hat{\mathbf{y}}$ of $\mathbf{y}$ as $\hat{\mathbf{y}} = [y_1-0.5, y_2-0.5, \cdots]$.


%\begin{definition}[Residual Variable and Vector] 
%\label{def_1}
%We define the residual of a variable $y$ as $\hat{y}=y-0.5$; 
%and we define the residual vector $\hat{\mathbf{y}}$ of $\mathbf{y}$ as $\hat{\mathbf{y}} = [y_1-0.5, y_2-0.5, \cdots]$.
%and we define the residual matrix $\hat{\mathbf{Y}}$ of $\mathbf{Y}$  as each entry of $\mathbf{Y}$ substracting 0.5.
%\end{definition}




%\begin{lemma}[Residual Messages] The residual message $\hat{m}_{vu}^{(t)}$ can be represented as follows:
%\label{lemma_1}
%%With above denotation, we have
%\begin{equation}
%\small
%\label{res_nei_influ_sybil}
%\hat{m}_{vu}^{(t)} = 
%\begin{cases} 
%0 & \text{if } \hat{p}_v^{(t-1)}  > 0 \text{ and } v \in \Gamma_{i} (u) \\
%0 & \text{if } \hat{p}_v^{(t-1)}  < 0 \text{ and } v \in \Gamma_{o} (u) \\
%2 \hat{p}_{v}^{(t-1)} \hat{w} &\text{otherwise}.
%\end{cases} 
%\end{equation}
%\end{lemma}
%
%\begin{proof}
%By substituting variables in Eqn.~\ref{modifiedMessage} with their residuals.
%\end{proof}

%We denote by $\mathbf{A}_b\in \mathbb{R}^{|V| \times |V|}$, $\mathbf{A}_i\in \mathbb{R}^{|V| \times |V|}$, and $\mathbf{A}_o\in \mathbb{R}^{|V| \times |V|}$ the bidirectional, unidirectional incoming, and unidirectional outgoing adjacency matrices of the social graph, respectively. 
%The $u$th row of $\mathbf{A}_b$, $\mathbf{A}_i$, and $\mathbf{A}_o$ represents the bidirectional, unidirectional incoming, and unidirectional outgoing neighbors of $u$. Formally, if there exists a bidirectional edge between $u$ and $v$, then the entry $A_{b,uv}=A_{b,vu}=1$, otherwise, $A_{b,uv}=A_{b,vu}=0$;
%if there exists an unidirectional edge from $u$ to $v$, then $A_{o,uv}=1$ and $A_{i,vu}=1$.
 
For convenience, we denote by $\mathbf{p}^{(t)} = [p_1^{(t)} ; p_2^{(t)} ; \cdots; p_{|V|}^{(t)} ]$ a column vector all users' posterior probability in the $t$th iteration, and its residual vector as $\hat{\mathbf{p}}^{(t)} $. Similarly, we denote by a column vector $\mathbf{q}  = [q_1; q_2; \cdots; q_{|V|}]$ all users' prior probability,  and by $\hat{\mathbf{q}} $ its residual vector. Moreover, we denote by $\mathbf{M}\in \mathbb{R}^{|V| \times |V|}$ the adjacency matrix of the social graph. 
 %Let $\hat{\mathbf{P}}^{(t)} \in \mathbb{R}^{|V| \times |V|}$ be a matrix consisting of $|V|$ repeats of the column vector $\hat{\mathbf{p}}^{(t)} $, i.e., $\hat{\mathbf{P}}^{(t)}  = [\hat{\mathbf{p}}^{(t)} , \hat{\mathbf{p}}^{(t)} , \cdots]$. 
With these notations, we can approximate AttriInfer as a concise matrix form. Formally, we have the following theorem. 

%We define $\mathbf{p} = [p_1; p_2; \cdots; p_{|V|}]$ as the column vector of all nodes' posterior beliefs, and $\hat{\mathbf{p}}$ as its residual vector. Similarly, we denote by $\mathbf{q} = [q_1; q_2; \cdots; q_{|V|}]$ the column vector of all nodes' prior beliefs.  and by $\hat{\mathbf{q}}$ its residual vector. 
%
%With these notations and By setting all $w_{vu}$ as a fixed $w$, we have the following theorem regarding the approximate GANG.


% We further define $\mathbf{Q}=[\mathbf{q}_{1}; \mathbf{q}_{2}; \cdots ; \mathbf{q}_{|V|} ] = [\mathbf{q}(1), \mathbf{q}(-1)] \in \mathbb{R}^{|V| \times 2}$ and $\mathbf{P}=[\mathbf{p}_{1}; \mathbf{p}_{2}; \cdots ;  \mathbf{p}_{V}] = [\mathbf{p}(1), \mathbf{p}(-1)] \in \mathbb{R}^{|V| \times 2}$; their residual matrices are $\hat{\mathbf{Q}}=[\hat{\mathbf{q}}(1), \hat{\mathbf{q}}(-1)]$ and $\hat{\mathbf{P}}=[\hat{\mathbf{p}}(1),\hat{\mathbf{p}}(-1)]$. With such definitions, we have the following theorem regarding the approximate GANG.

\begin{theorem}
\label{theorem_1}
%Denote $\mathbf{A} \circ \mathbf{B}$ as the Hadamard (element-wise) product of matrix $\mathbf{A}$ and $\mathbf{B}$. 
%Furthermore, we set $\hat{\mathbf{p}}^{(0)} = \hat{\mathbf{q}}$. 
We can approximate Equations.~\ref{modifiedMessage} and~\ref{belief}  as the following equation: 
%the final residual belief vector $\hat{\mathbf{p}}$ can be approximated by iteratively solving the following equations
\begin{equation}
\label{approx_update}
\hat{\mathbf{p}}^{(t)} = \hat{\mathbf{q}} + 2\cdot\hat{w}\cdot \mathbf{M} \cdot \hat{\mathbf{p}}^{(t-1)}.
\end{equation}
%where the operator $\circ$ represents element-wise product of two matrices, $\mathbf{Y}^T$ is the transpose of the matrix $\mathbf{Y}$, and the indicator function $I(\mathbf{Y})$ means that an entry is set to be 0 if the corresponding entry of the matrix $\mathbf{Y}$ is non-negative, otherwise it is set to be 1. 
%  means setting positive entries of matrix $\mathbf{Y}$ to be 0, and $\mathbf{Y}(\mathbf{Y}<0)=0$ means setting negative entries of matrix $\mathbf{Y}$ to be 0. 
\end{theorem}
\begin{proof}
See Appendix~\ref{app:theorem1}.
\end{proof}

Theorem~\ref{theorem_1} enables us to design an efficient version of AttriInfer: first, we learn the prior probability for each user using behaviors; second, we iteratively apply Equation~\ref{approx_update} to compute the posterior probabilities for all target users simultaneously. AttriInfer halts when the relative change of the posterior probability vector in two consecutive iterations is smaller than $10^{-3}$.

We note that Gatterbauer et al.~\cite{gatterbauer2015linearized} also linearized LBP over a pMRF, and their linearized version is similar to ours. However, their linearization requires different heuristics and assumptions. For instance, their linearization requires residual of the homophily strength to be very small and the approximation of $\frac{\frac{1}{k}+\epsilon_1}{1+\epsilon_2}\approx \frac{1}{k} +\epsilon_1 -\frac{\epsilon_2}{k}$ when $\epsilon_1$ and $\epsilon_2$ are very small. In contrast, our linearization does not require these assumptions/approximations. Moreover, we eliminate message maintenance before linearizing Equation~\ref{belief}, which makes linearization much simpler, while their approach does not.

 
%demonstrates that posterior beliefs can be iteratively solved by matrix operations without explicitly modeling messages. 
%\textbf{Algorithm 2} summarizes our optimized version of GANG (GANG\_Opt). We note that Gatterbauer et al.~\cite{gatterbauer2015linearized} linearized LBP for a standard pMRF modeling an undirected graph, 
%while our work linearizes LBP for a new pMRF modeling a directed graph. 

%Note that above update equations directly calculate beliefs, i.e., without storing the passing messages. Moreover, the update can converge after several iterations (See Section VI). In doing so, we then predict $u$ to be a fraudulent node if $\hat{p}_u(1) > 0 $. For simplicity, we denote such approximate GANG as GANG\_Appr and illustrate its algorithmic procedure in \textbf{Algorithm 2}. 

%\begin{algorithm}[!htb]
%\caption{Optimized version of GANG (GANG\_Opt)}
%\label{alg:GANG}
%\begin{algorithmic}
%\REQUIRE $G=(V,E)$, $L_f$, $L_n$, $\epsilon$, $w$, $\delta=10^{-3}$, and $T=20$. \\
%\ENSURE  $p_u, \forall \, u \in V$. \\
%    Initialize $\hat{\mathbf{p}}^{(0)} = \hat{\mathbf{q}}$. \\
%    Initialize $t=1$. \\
%%\noindent \textbf{Process:}
%%\PROCESS ~~\\
%    %\WHILE { $\sum_{u\in V}|\hat{{p}}_u^{(t)} - \hat{{p}}_u^{(t-1)}| \geq \delta$ and $t \leq T$} \;
%    \WHILE { $\frac{\|\hat{\mathbf{p}}^{(t)} - \hat{\mathbf{p}}^{(t-1)}\|_1} {\|\hat{\mathbf{p}}^{(t)}\|_1} \geq \delta$ and $t \leq T$} \;
%    \STATE Update residual belief vector $\hat{\mathbf{p}}^{(t)}$ using Eqn.~\ref{approx_update}; \\
%    \STATE  $t=t+1$. \\
%    \ENDWHILE \\
%    \RETURN $\hat{\mathbf{p}}^{(t)} + 0.5$. \\
%\end{algorithmic}
%\end{algorithm}

 
 
 \section{Theoretical Analysis}
 \subsection{Convergence Analysis}
\label{sec:cvgAnal}
We analyze the condition when the optimized version of AttriInfer converges. Such analysis guides us to select appropriate homophily strength $w$.
Suppose we are given an iterative linear process: $\mathbf{y}^{(t)} \leftarrow \mathbf{c} + \mathbf{D} \mathbf{y}^{(t-1)}$. 
According to~\cite{saad2003iterative}, the linear process converges with any initial choice $\mathbf{y}^{(0)}$ if and only if the \emph{spectral radius} of the matrix $\mathbf{D}$ is smaller than 1, i.e., $\rho(\mathbf{D}) < 1$. The spectral radius of a square matrix is the maximum of the absolute values of its eigenvalues.
Given this general result, we are able to analyze the convergence condition of AttriInfer.  

\begin{theorem}[Sufficient and Necessary Condition] 
\label{lemma_2}
The sufficient and necessary condition that AttriInfer converges is to bound 
the residual homophily strength $\hat{w}$ as:  
\begin{align}
\label{suff_ness_cond}
\begin{split}
 \hat{w} < \frac{1}{2 \rho(\mathbf{M})}.
\end{split}
\end{align}

\end{theorem}
\begin{proof}
Let $\mathbf{D} = 2\hat{w} \cdot \mathbf{M}$, then $\rho(\mathbf{D})= 2\hat{w} \cdot \rho(\mathbf{M})$.  $\rho(\mathbf{D})< 1$ holds if and only if $\hat{w} < \frac{1}{2\rho (\mathbf{M})}$.
%See Appendix~\ref{app:prooflemma2}.
\end{proof}

Theorem~\ref{lemma_2} provides a strong sufficient and necessary convergence condition.
However, in practice setting $\hat{w}$ using Theorem~\ref{lemma_2} is computationally expensive, as it involves computing the largest eigenvalue with respect to spectral radius. Hence, we instead derive a \emph{sufficient condition} for AttriInfer's convergence, which enables us to set $\hat{w}$  with cheap computation. Specifically, our sufficient condition is based on the fact that any norm is an upper bound of the spectral radius~\cite{derzko1965bounds}, i.e., $\rho(\mathbf{D}) \leq \| \mathbf{D} \|$, where $\| \cdot \|$ indicates some matrix norm. 
In particular, we use the induced $l_1$ matrix norm $\| \cdot \|_1$, where $\| \mathbf{D} \|_1 = \max_{j } \sum_{i} | \mathbf{D}_{ij} | $, the maximum absolute column sum of the matrix. In this way, our sufficient condition for convergence is as follows:

\begin{theorem}[Sufficient Condition] 
\label{lemma_3}
The sufficient condition that AttriInfer converges is
\begin{align}
\label{suff_cond}
\hat{w} < \frac{1}{2\| \mathbf{M} \|_1}=\frac{1}{2\max_{u \in V} d_u}, 
\end{align}
where $d_u=|\Gamma_u|$ is the degree of $u$.
%where $d_u=|\Gamma_u|$ is the number of neighbors of $u$.
\end{theorem}
\begin{proof}
As $\rho(\mathbf{D}) \leq \|\mathbf{D}\|_1$, we achieve the sufficient condition by enforcing $\|\mathbf{D}\|_1 < 1$, where $\mathbf{D} = 2\hat{w} \cdot \mathbf{M}$. Specifically, we have
\begin{align} 
2\hat{w} \cdot \rho(\mathbf{M})  < 1 \Longleftarrow & 2 \hat{w} \|{\bf M}\|_1 < 1 \\
 \Longleftarrow & \hat{w} < \frac{1}{2 \|\mathbf{M}\|_1} = \frac{1}{2 \max_{u\in V} d_u}.
%$2\hat{w} \cdot \rho(\mathbf{A}) \leq 2\hat{w} \|\mathbf{M}\|_1 < 1 \rightrightarrow \hat{w} < \frac{1}{2 \|\mathbf{M}\|_1} = \frac{1}{2 \max_{u\in V} D_u}.$
%See Appendix~\ref{app:prooflemma3}.
\end{align}
\end{proof}

Theorem~\ref{lemma_3} guides us to set $\hat{w}$, i.e., once $\hat{w}$ is smaller than the inverse of 2 times of the maximum node degree, AttriInfer is guaranteed to converge. 
In practice, however, some users (e.g., celebrities) could have orders of magnitude bigger degrees than the others (e.g., ordinary people), and such nodes make $\hat{w}$ very small. 
In our experiments, we find that AttriInfer can still converge when replacing the maximum node degree with the average node degree.

 \subsection{Complexity Analysis}
  We use sparse matrix representation to implement AttriInfer. 
 Computational time of the optimized AttriInfer consists of two parts: time required to compute the prior probabilities using logistic regression, 
 and time required to compute the posterior probabilities via iterative computations.  
The time complexity of the second part is $O(t \cdot |E|)$, where $t$ is the number of iterations.
The time complexity of AttriInfer does not rely on the number of target users whose attributes an attacker wants to infer. 
 We note that the basic version of AttriInfer has the same asymptotic time complexity. 
 However, the constants in the asymptotic representations are different, 
 which results in different scalability. 
 
 VIAL~\cite{GongAttributeInfer16} does not learn the prior probabilities. For each target user, VIAL 
 computes the stationary probability distribution of a random walk in the augmented graph, which starts from the target user. 
 The time complexity of VIAL is $O(t \cdot (|E| + m_1 + m_2) \cdot n_t)$, where $t$ is the number of iterations that a random walk requires to converge, 
 $m_1$ is the total number of public attributes of all users, $m_2$ is the total number of behaviors of all users, and $n_t$ is the number of target users. 
 As we will demonstrate in our experiments, although VIAL does not learn the prior probabilities, it will be orders of magnitude slower than AttriInfer when 
 an attacker aims to infer attributes for a large number of target users. 


==> related-old.tex <==

\section{Background and Related Work}
\label{relatedwork}

\subsection{Frequency Estimation with LDP}
Suppose we have $d$ items (denoted as $\{1,2,\cdots,d\}$) and $n$ users. Each user has a single item.   
A data collector aims to compute the frequency $c_i$ of each item among the $n$ users, i.e., $c_i$ is the number of users that have the item $i$.  
%An item is an answer to a certain question asked by the data collector. 
For instance,  an item is Yes or No when the data collector is interested in estimating the number of users that are HIV positive and negative in a survey; 
an item is a webpage when the data collector (e.g., Google) aims to estimate the number of users that set a webpage as a browser's default homepage; an item is a feature of a mobile app when the data collector (e.g., the app developer) aims to estimate the number of users that use each feature. Frequency estimation enables the data collector to further perform other advanced data analytics (e.g., heavy hitter estimation, frequent itemset mining), improve services to users, optimize client software (e.g., mobile apps), and detect unwanted or malicious hijacking of user settings in browsers~\cite{Erlingsson:2014,Ninghui:2017}. 

%question is ``are you HIV positive?"; an item is a webpage when the question is ``what is your browser's default homepage"; and an item is a search engine when the question is ``what is your default search engine". 
%
%a webpage a user clicks or visits, or the default homepage of a user's browser.    default

A naive solution for frequency estimation is to ask each user to share its item with the data collector, who can compute the items' frequencies easily. However, this naive solution faces two challenges. First, when the items are sensitive, users may not be willing to share their raw items with the data collector. Second, the data collector could be compromised to leak the users' items, which frequently happens in real world, e.g., Equifax was recently compromised and personal data of 143 million users were leaked~\cite{}.  

Local differential privacy (LDP)~\cite{}, a privacy protection mechanism based on $\epsilon$-differential privacy~\cite{Dwork:2006}, can address the challenges. In LDP, a user's item is perturbed according a randomized algorithm $\mathcal{A}$ before sending to the data collector. 
LDP is formally defined as follows:

%The algorithm  $\mathcal{A}$ satisfies $\epsilon$-local differential privacy with the following definition:

\begin{definition}[{\bf Local Differential Privacy}]
A randomized algorithm $\mathcal{A}$ is said to satisfy $\epsilon$-local differential privacy (LDP) if and only if for any items $i$ and $j$, we have
\begin{align}
%\textbf{Privacy-utility tradeoff } & \textbf{with a privacy-risk budget:} \nonumber \\
\forall t \in Output(\mathcal{A}),  \frac{Pr(\mathcal{A}(i)=t)}{Pr(\mathcal{A}(j)=t)} \leq e^\epsilon,
\end{align}
where $\epsilon\geq 0$ and $Output(\mathcal{A})$ is the set of all possible outputs of the randomized algorithm $\mathcal{A}$.
\end{definition}
  
Roughly speaking, in LDP, any two items have close probabilities to be perturbed to the same item. The data collector receives a perturbed item from each user and aims to estimate item frequencies from the perturbed items. Next, we discuss state-of-the-art LDP algorithms to perturb items and estimate item frequencies. 


%Differential Privacy~\cite{Dwork:2008,Dwork:2006} is the state-of-the-art data perturbation technique to protect users' privacy when the data collector is trustful. However, the data collector may be compromised or the data collector itself is unbelievable in real scenarios. Also, data collector will take responsibility for the protecting of users' privacy which may trap the data collector into dilemma and thus, resulting in the unwillingness of data collector to collect users' data. If the data collector also can't access the actual data of users, the above concerns would be solved. An intutive solution is that each user perturb her data locally bofore sending the data to the data collector. Local Differential Privacy (LDP)~\cite{Ninghui:2017,Blender:2017,QinHeavyHitterCCS16,Erlingsson:2014,FantiBuildRappor,BassilySuccinctHistograms15} is a recently developed technique based on this and has been deployed by Google, Apple. For example, Google has implemented RAPPOR~\cite{Erlingsson:2014,FantiBuildRappor} in Google Chrome browser to collect webpages that user click. Apple also claims that they have used Differential Privacy~\cite{AppleDP} to protect user privacy but the algorithm details haven't been published. 
%
%Here we will give an overview of LDP protocols. As a simplification, assume each user hold one item, for example, the webpage that user click. Users will add some noise before sending the data to the data collector. For example, user may randomly report some webpages with some probability. When the data collector receives those noisy data, she can perform some analysis towards the noisy data. One important analysis is the histogram estimation, that is, the data collector need to estimate the number of users for each item. For example, Google can estimate how many users have looked through a certain webpage after receiving reported data from Google Chrome. And the result will be used to improve search quality to provide better search experience to users. Thus, it is fairly important to accurately estimate the count of each items. In the next, we will formally discuss LDP. 


%\begin{definition}\hspace{-1mm}[{\bf Differential Privacy}]
%A mechanism $\mathcal{M}$ is said to satisfy $\epsilon$-Differential Privacy($\epsilon \geq 0$) iff for any two adjacent databases $D$ and $D^{\prime}$, we have
%\begin{align}
%\textbf{Privacy-utility tradeoff } & \textbf{with a privacy-risk budget:} \nonumber \\
%\forall t \in Output(\mathcal{M}),  \frac{Pr(\mathcal{M}(D)=t)}{Pr(\mathcal{M}(D^\prime)=t)} \leq e^\epsilon
%\end{align}
%where $Output(\mathcal{M})$ is a set which contains all the possible output of algorithm $\mathcal{M}$.
%\end{definition}

\subsection{Local Differential Privacy Algorithms}
The first LDP algorithm called \emph{randomized response} dates back to 19XXs~\cite{}. Recently, several LDP algorithms~\cite{} were proposed, e.g., RAPPOR~\cite{}, Optimized Unary Encoding (OUE)~\cite{}, XX~\cite{}.  XX~\cite{} summarized that all existing LDP algorithms essentially consist of three steps, i.e., \textbf{Encode}, \textbf{Perturb}, and \textbf{Aggregate}. In the {Encode} step, a LDP algorithm encodes a user's categorical data item into a numerical value or a vector; in the {Perturb} step, a LDP algorithm perturbs a user's encoded value or vector such that local differential privacy is achieved; in the {Aggregate} step, the data collector estimates item frequencies from the perturbed encoded values or vectors from all users. The Encode and Perturb steps are performed at client side for every user, while the {Aggregate} step is performed at the data collector side.  

Moreover, state-of-the-art LDP algorithms (e.g., OUE, XX, XX, XX) satisfy \emph{pure local differential privacy}, which is formally defined as follows:
\begin{definition}[{\bf Pure Local Differential Privacy}]
A randomized algorithm $\mathcal{A}$ with the $Encode$ and $Perturb$ steps is pure local differential privacy if and only if there exists two probability values $p^*$ and $q^*$ such that for all item  $i$.
\begin{align}
%\textbf{Privacy-utility tradeoff } & \textbf{with a privacy-risk budget:} \nonumber \\
&Pr[Perturb(Encode(i)) \in \{y|i\in Support(y)\}]=p^*, \\
\forall_{j\neq i}&Pr[Perturb(Encode(j)) \in \{y| i \in Support(y)\}]=q^*,
\end{align}
where $Support(y)$ is the set of items that an output $y$ supports. 
\end{definition}
For any pure LDP algorithm, the data collector can use the following equation to estimate item frequencies in the Aggregate step~\cite{}:
\begin{align}
\label{agg}
\hat{c}_i=\frac{\sum_{u}\mathbbm{1}_{Support(y_u)}(i)-nq^*}{p^*-q^*},
\end{align}
where $y^u$ is the perturbed encoded output of user $u$; the function $\mathbbm{1}_{Support(y_u)}(i)$ is 1 if $y^u$ supports the item $i$, otherwise it is 0. Intuitively, for every perturbed encoded output from users, we add one count to the items that are supported by the output. In the end, we normalize the counts using the probabilities $p^*$ and $q^*$. Different pure LDP algorithms use different Encode steps and/or Perturb steps, and thus they have different Support functions, $p^*$, and $q^*$.  Next, we will review two representative pure LDP algorithms XX and XX that were recently proposed by XX et al.~\cite{}. XX and XX have the same frequency estimation errors. Compared with XX, XX has a lower communication cost between users and data collector, but it has a higher computational cost for the data collector. 

 

\subsubsection{Optimized Unary Encoding (OUE)}
OUE is an optimized version of the basic RAPPOR algorithm proposed by Erlingsson et. al.~\cite{Erlingsson:2014}. 

\myparatight{Encode} OUE uses \emph{unary encoding} to encode an item. Specifically, OUE uses a length-$d$ binary vector $\mathbf{X}$ to encode the $d$ items. If a user has item $i$, then $\mathbf{X}[i]=1$ and all other entries of $\mathbf{X}$ are 0.   

\myparatight{Perturb} In this step, OUE perturbs a binary vector $\mathbf{X}$ into another binary vector $\mathbf{Y}$ probabilistically bit by bit. Specifically, we have:
\begin{align}
\label{oueperturb}
Pr(\mathbf{Y}[i]=1)=\left \{ 
\begin{aligned}
p=&\frac{1}{2}, \text{ if }\mathbf{X}[i]=1 \\
q=&\frac{1}{1+e^{\epsilon}}, \text{ if }\mathbf{X}[i]=0 
\end{aligned}
\right.
\end{align}
If a bit in $\mathbf{X}$  is $1$, then the corresponding bit in $\mathbf{Y}$ will be 1 with a probability $\frac{1}{2}$. However, if a bit in $\mathbf{X}$  is $0$, then the corresponding bit in $\mathbf{Y}$ will be 1 with a  probability $\frac{1}{1+e^{\epsilon}}$ that is smaller than $\frac{1}{2}$. 

\myparatight{Aggregate} Once the data collector receives the perturbed binary vectors $\mathbf{Y}$ from users, the data collector estimates the frequency $\hat{c}_i$ of item $i$ using Equation~\ref{agg} with the function $\mathbbm{1}_{Support(y_u)}(i)=\mathbf{Y}_{u}[i]$, $p^*=p$, and $q^*=q$, where $\mathbf{Y}_{u}$ is the perturbed binary vector from user $u$. 

%she can perform unbiased estimation of the frequency of each item. Here we use $j$ to denote the user index and $Y_{j}$ denote the noisy vector received from user $j$. The count of item $i$ can be estimated by the following equation.
%\begin{align}
%\hat{c}(i)=\frac{\sum_{j}\mathbf{Y}_{j}[i]-nq}{p-q}
%\end{align}


%The main drawback of Basic RAPPOR and OUE is high communication cost, that is, each user need to transmit $d$ bits to data collector which is very high when $d$ is very large. For example, if the item domain is the webpage, then $d$ is the total number of webpage which leads to unaccptable communication cost. 

\subsubsection{Optimal Local Hashing (OLH)} 
OLH leverages hash functions  hash the input value into the range $\{0,1,...,g-1\}$ by using a randomly chosen hash function $H$ from universal hash function family $\mathcal{H}$. The client only need to transmit the index of hash function being used as well as the output of hash function. OLH extends from Binary Local Hash (BLH) which essentially equivalent to the matrix-based protocol proposed in~\cite{BassilySuccinctHistograms15}. In BLH, the output of hash function is one bit which loses a lot of information about input. Thus, OLH uses more bits to encode the input at the price of more information loss in the perturb process. The trade-off between encode and perturb makes it possible to find optimal $g$ which is $e^{\epsilon}+1$. 

\myparatight{Encode} $y=H(X)$, $H \in \mathcal{H}$. The output is $\{index_{H},y\}$ where $index_{H}$ is the index of $H$ in hash family $\mathcal{H}$. 

\myparatight{Perturb} The perturb of the $y$ is as follows


\begin{align}
\forall_{i \in [g]}Pr(y=i)=\left \{ 
\begin{aligned}
p=&\frac{e^{\epsilon}}{g-1+e^{\epsilon}}, \text{if }x=i \\
q=&\frac{1}{g-1+e^{\epsilon}}, \text{if }x \neq i 
\end{aligned}
\right.
\end{align}

\myparatight{Aggregate} The aggregate of the OLH is as follows:

\begin{align}
\hat{c}(i)=\frac{\sum_{j}1_{y_{j}=H(i)}-nq}{p-q}
\end{align}

Compared with OUE, OLH significantly reduce the communication cost which is $\log m+ \log g$ where $m$ is the number of hash function. However, OLH need to compute the hash function which makes it is harder to implement in client and incur extra computation costs. Thus, when the communication cost $d$ is acceptable, OUE is a good choice because its both easy to implement and accurate in histogrm estimation. However, when domain size $d$ is large, OLH is a good choice because it has relative low communication cost.  
 



Local Differential Privacy (LDP)~\cite{Ninghui:2017,Blender:2017,QinHeavyHitterCCS16,Erlingsson:2014,FantiBuildRappor,BassilySuccinctHistograms15} refers to the privacy preserving data collecting framework based on $\epsilon$-Differential Privacy. Before we come to the definition of LDP. We will first give an intutive explanation of Differential Privacy. Differential Privacy is originally proposed to publish statistics data of users' database such that adversary can't infer with high probability of whether a user is in the database or not. Specifically, assuming there are two databases $D$ and $D^\prime$ and there is just one entry that is different. We use $\mathcal{M}$ to denote the perturb mechanism that satisfies $\epsilon$-Differential Privacy. Then, given the output $t$ of mechanism $\mathcal{M}$, we can't infer with high probability whether the input is $D$ or $D^\prime$. Thus, $\epsilon$-Differential Privacy provides possible deniability of whether a user is in the database or not. The $\epsilon$ is the mechanism parameter called \emph{Privacy Budget} which is used to control the strength of privacy protection. Compared with $\epsilon$-Differential Privacy, in LDP, each user perturb her data locally and satisfies $\epsilon$-Differential Privacy. In this situations, we can look $D$ and $D^\prime$ as databases that contains only one entry or look $D$ and $D^\prime$ as different items. As we can see, $D$ and $D^\prime$ differ in one entry from either perspective. In this paper, we assume $D$ and $D^\prime$ denote different items. Each user will send perturbed data to the data collector and the data collector would perform some analysis towards those noisy data. In this paper, we focus on histogrm estimation~\cite{BassilySuccinctHistograms15} which can be further used for other application, like heavy hitter~\cite{QinHeavyHitterCCS16}. LDP offers a more strong protection towards users' privacy because only the user knows the actual data and data collector can only access perturbed data.  

Generally, we assume there are $d$ items. Each user $u$ holds one item and we use $v$ to denote its index. Each user would perturb her data locally before sending the data to the data collector and we use $t$ to denote the output of users' perturb algorithm $\mathcal{M}$. The perturb algorithm $\mathcal{M}$ satisfies local differential privacy with the following definition:

\begin{definition}\hspace{-1mm}[{\bf Local Differential Privacy}]
A mechanism $\mathcal{M}$ is said to satisfy $\epsilon$-Local Differential Privacy($\epsilon \geq 0$) iff for any two possible input values $v$ and $v^{\prime}$, we have
\begin{align}
%\textbf{Privacy-utility tradeoff } & \textbf{with a privacy-risk budget:} \nonumber \\
\forall t \in Output(\mathcal{M}),  \frac{Pr(\mathcal{M}(v)=t)}{Pr(\mathcal{M}(v^\prime)=t)} \leq e^\epsilon
\end{align}
where $Output(\mathcal{M})$ is a set which contains all the possible output of algorithm $\mathcal{M}$.
\end{definition}

There are a variety of mechanisms that satisfy $\epsilon$-Differential Privacy have been developed. However, many of them require to access all users' data. In LDP, each user runs the mechanism independently such that each user only access her own data which makes mechanisms designed for $\epsilon$-Differential Privacy can't apply to LDP. Although some fundamental mechanisms such as Laplace Mechanism~\cite{Dwork:2008} can be applied to LDP, however, it suffers sub-optimal privacy-utility trade-off.

Several LDP protocols~\cite{Ninghui:2017,Erlingsson:2014,BassilySuccinctHistograms15,shaoweiwang16} have been developed by multiple research communities such as RAPPOR, OUE and OLH. Basically, for each protocol, there are three steps: \textbf{Encode}, \textbf{Perturb} and \textbf{Aggregate} in which \textbf{Encode} and \textbf{Perturb} is executed by user locally while \textbf{Aggregate} is exectuted by data collector. Specifically, $\textbf{Encode}$ is being used to encode the items. $\textbf{Perturb}$ output the perturbed data which satisfies $\epsilon$-LDP to protect users' privacy.  $\textbf{Perturb}$ is highly related to the encode methods. $\textbf{Aggregate}$ is executed by data collector to estimate the frequency of each item.

\myparatight{Encode} The algorithm output encoded value $X$ given the input value $v$, that is, $X=Encode(v)$. 

\myparatight{Perturb} The algorithm output perturbed value $Y$ given the input $X$, that is, $Y=Perturb(X)=Perturb(Encode(v))$. 


\myparatight{Aggregate} The algorithm output the frequency of each item after reveiving perturbed data $Y$ from all users.

%Different protocols have different encoding strategies which result in different communication cost as well as different perturb methods. 
%There are several protocols~\cite{Ninghui:2017,Erlingsson:2014,BassilySuccinctHistograms15,shaoweiwang16} have been developed by multiple research communities. 
%Li et. al.~\cite{Ninghui:2017} propose a framework named "pure" Local Differential Privacy Protocols (Pure-LDP-Protocols) which could be used to analyze %different LDP protocols and optimize parameter setting of different protocols. Following this framework, we catogerize the existing LDP protocols into %two class: Pure-LDP and Non-pure LDP.

In the next, we will study three examples of existing LDP protocols: Basic RAPPOR, OUE and OLH. OUE is optimized Basic RAPPOR. Specifically, the difference between Basic RAPPOR and OUE is the parameter setting in $\mathbf{Perturb}$ and OUE is more accurate in estimating the frequency of each item given the same privacy budget. Thus, we mainly focus on OUE and OLH which is state-of-the-art LDP protocols in terms of estimation accuracy. Because OUE and Basic RAPPOR use the same $\mathbf{Encode}$ method, thus, OUE has the same communication cost with Basic RAPPOR which is the number of items. OLH uses local hash to encode items which can decrease the communication cost. Thus, when the number of items is large, OUE and Basic RAPPOR has relatively big communication cost compared with OLH which makes OLH a good choice. However, OLH needs to compute hash function in client which makes it is hard to implement and also incur extra computation burden to both client and server. Thus, when the communcation cost of OUE is acceptable, OUE is a good choice for its simplicity and low computation cost. 
\subsection{Three Examples of LDP Protocols}

%Before we come to the specific Pure-LDP-Protocols, we will formally give the definition of Pure-LDP-Protocols. 
%\begin{definition}\hspace{-1mm}[{\bf Pure LDP Protocols}]
%A protocol given the $Encode$ and $Perturb$ as well as the $Support$ function is pure iff there exist two probability values $p^*$ and $q^*$ such that %for all input values $v_{1}$.
%\begin{align}
%\textbf{Privacy-utility tradeoff } & \textbf{with a privacy-risk budget:} \nonumber \\
%&Pr[Perturb(Encode(v_{1}))] \in \{y|v_{1}\in Support(y)\}=p^*, \\
%\forall_{v_{2}\neq v_{1}}&Pr[Perturb(Encode(v_{2}))] \in \{y|v_{1}\in Support(y)\}=q^*
%\end{align}
%where $Support$ function maps each possible output value $y$ into the possible input values that $y$ "support".
%\end{definition}

%Li et. al.~\cite{Ninghui:2017} also provides an unbiased aggregation strategy for Pure-LDP-Protocols. There is a simple aggregation technique to compute the number of each item under this framework.

%Different encode function lead to different communication cost. A large encode length usually contains more information about the input value. 
%Different Pure-LDP-Protocols have different encode function and perturb method. 
%There is an unbiased estimation given $p^*$ and $q^*$ for Pure-LDP-Protocols. 
%For a pure LDP protocol, let $y^j$ denote the noisy value sent by user $j$, $\hat{c}(i)$ denote the estimated number of item $i$. Then, the unbiased %estimation of item $i$ is:

%\begin{align}
%\hat{c}(i)=\frac{\sum_{j}\mathbbm{1}_{Support(y^j)}(i)-nq^*}{p^*-q^*}
%\end{align}
 

\subsubsection{Basic RAPPOR}

Erlingsson et. al.~\cite{Erlingsson:2014} proposes Basic RAPPOR which extends random response (RR). RR is a commonly used technique to protect users' privacy when conducting surveys involving private information. Specifically, assuming we conduct a survey which we want to know the percentage of homosexuality in a population. However, if we directly ask the participants "Are you homosexual or not?". The participants may not willing to provides the true answer if he or she is homosexual especially in the culture not friend to the homosexual. RR can be used to solve this problem by providing deniability for a user towards his answer. More specifically, each user flips a biased coin before answering the question. If the coins turn head (with probability $p$), the participants provide right answer, otherwise, participants provide the opposite of the right answer. The data collector can compute an unbiased estimation after receiving those noisy data from users. Basic RAPPOR also uses RR to perturb the encoding vector bit by bit.

%~\cite{Erlingsson:2014} has proven that Random Response satisfies $\epsilon$-Local Differential Privacy with the following probability $p$.



%Intutively, Basic RAPPOR uses length-$d$ bit binary vector to encode the items. and perturbs vector bit by bit with some probability and sends the perturbed vector to the data collector. 
\myparatight{Encode} The Basic RAPPOR use length-$d$ binary vector $\mathbf{X}$ to encode $d$ items whose bits are all zero except the one bit indexed by $v_{j}$ which is the item hold by user $j$. 

\myparatight{Perturb} 
%The perturb of the Basic RAPPOR
%holds one item $v_{i}$. The Basic RAPPOR use length-$d$ binary vector $\mathbf{X}$ to encode $d$ items whose bits are all zero except the one bit indexed by $v_{i}$. Each user perturbs the encoding vector $\mathbf{X}$ bit by bit with same probability and sends the result $\mathbf{Y}$ to the data collector. 
~\cite{Erlingsson:2014} use the following ways to perturb the $\mathbf{X}$ bit by bit and proves that it satisfies the $\epsilon$-Local Differential Privacy.
\begin{align}
Pr(\mathbf{Y}[i]=1)=\left \{ 
\begin{aligned}
p=\frac{e^{\frac{\epsilon}{2}}}{1+e^{\frac{\epsilon}{2}}}, \text{if }\mathbf{X}[i]=1 \\
q=\frac{1}{1+e^{\frac{\epsilon}{2}}}, \text{if }\mathbf{X}[i]=0 
\end{aligned}
\right.
\end{align}

As we can see, for each bit in encoding vector, its value will be kept with probability $p$ and reversed with probability $q$. This perturb process treat $0$ and $1$ equally, that is, no matter what value it is in encoding vector, the perturb process is the same. 

\myparatight{Aggregate} Once the data collector receives the noisy data from users, she can perform unbiased estimation of the frequency of each item. Here we use $j$ to denote the user index and $Y_{j}$ denote the noisy vector received from user $j$. The count of item $i$ can be estimated by the following equation.
\begin{align}
\hat{c}(i)=\frac{\sum_{j}\mathbf{Y}_{j}[i]-nq}{p-q}
\end{align}

\subsubsection{OUE}
As we have mentioned before, Basic RAPPOR treat $1$ and $0$ equally, that is, $p+q=1$. However, most of entries ($d-1$) in the encode vector are $0$ while only one bit is $1$. Wang et. al.~\cite{Ninghui:2017} optimzes the parameter to minimize the estimation variance and suggests an alternative ways to set the value of $p$ and $q$. Intutively, instead assigning the privacy budget $\epsilon$ to transmit $0$ and $1$ equally which is $\frac{\epsilon}{2}$ respectively in Basic RAPPOR, OUE assign all privacy budget $\epsilon$ to transmit $0$ which is main source of estimation variance. The OUE has the same encode and aggregation methods with the Basic RAPPOR. However, OUE is more accurate compared with Basic RAPPOR. We will use OUE rather than Basic RAPPOR since the only different between them is the parameter setting. 
\begin{align}
\label{oueperturb}
Pr(\mathbf{Y}[i]=1)=\left \{ 
\begin{aligned}
p=&\frac{1}{2}, \text{if }\mathbf{X}[i]=1 \\
q=&\frac{1}{1+e^{\epsilon}}, \text{if }\mathbf{X}[i]=0 
\end{aligned}
\right.
\end{align}


Equation~\ref{oueperturb} is the perturb of OUE. As we can see from the equation, if the bit in encoding vector is $1$, it will be kept with probability $\frac{1}{2}$. However, if the bit in encoding vector is $0$, its value will be kept with relative high probability which is $\frac{e^{\epsilon}}{1+e^{\epsilon}}$. 

The main drawback of Basic RAPPOR and OUE is high communication cost, that is, each user need to transmit $d$ bits to data collector which is very high when $d$ is very large. For example, if the item domain is the webpage, then $d$ is the total number of webpage which leads to unaccptable communication cost. 

\subsubsection{OLH} %~\cite{BassilySuccinctHistograms15} proposes a random matrix-based protocol which uses a random projection as encode function. Then, it use random response to perturb the encoding vector which satisfies $\epsilon$-Local Differential Privacy. Finally, this protocols output one random selected bit from the perturbed vector. 
%Li et. al.~\cite{Ninghui:2017} points out that this process is essentially a local hashing encoding which output one bit given input value. Li et. al. propose Binary Local Hashing (BLH) protocol which is logically equivalent to the above protocol. The BLH random chooses one hash function from universal hash function family $\mathbb{H}$ in which each hash function $H \in \mathbb{H}$ hashes an input value into one bit, that is, $b=H(v)$. Then, the user perturb $b$ and send the result $b^\prime$ as well as the hash function used to the data collector. 
Wang et. al.~\cite{Ninghui:2017} proposes Optimal Local Hash (OLH) which hash the input value into the range $\{0,1,...,g-1\}$ by using a randomly chosen hash function $H$ from universal hash function family $\mathcal{H}$. The client only need to transmit the index of hash function being used as well as the output of hash function. OLH extends from Binary Local Hash (BLH) which essentially equivalent to the matrix-based protocol proposed in~\cite{BassilySuccinctHistograms15}. In BLH, the output of hash function is one bit which loses a lot of information about input. Thus, OLH uses more bits to encode the input at the price of more information loss in the perturb process. The trade-off between encode and perturb makes it possible to find optimal $g$ which is $e^{\epsilon}+1$. 

\myparatight{Encode} $y=H(X)$, $H \in \mathcal{H}$. The output is $\{index_{H},y\}$ where $index_{H}$ is the index of $H$ in hash family $\mathcal{H}$. 

\myparatight{Perturb} The perturb of the $y$ is as follows


\begin{align}
\forall_{i \in [g]}Pr(y=i)=\left \{ 
\begin{aligned}
p=&\frac{e^{\epsilon}}{g-1+e^{\epsilon}}, \text{if }x=i \\
q=&\frac{1}{g-1+e^{\epsilon}}, \text{if }x \neq i 
\end{aligned}
\right.
\end{align}

\myparatight{Aggregate} The aggregate of the OLH is as follows:

\begin{align}
\hat{c}(i)=\frac{\sum_{j}1_{y_{j}=H(i)}-nq}{p-q}
\end{align}

Compared with OUE, OLH significantly reduce the communication cost which is $\log m+ \log g$ where $m$ is the number of hash function. However, OLH need to compute the hash function which makes it is harder to implement in client and incur extra computation costs. Thus, when the communication cost $d$ is acceptable, OUE is a good choice because its both easy to implement and accurate in histogrm estimation. However, when domain size $d$ is large, OLH is a good choice because it has relative low communication cost.  
 
\subsection{Insufficiency of Existing LDP Protocols}
All existing LDP protocols output the estimation result of last step: $\mathbf{Aggregate}$. However, this is noisy results. More specifically, the output of existing LDP protocols equals to the true value plus the noise sampled from the distribution of noise. For example, for Basic RAPPOR, its aggregation result for each item is the true count of that item plus the noise sampled from normal distribution. Based on this, we add another step: $\mathbf{Calibrate}$ to somehow "denoise" to makes the estimation more accurate of existing LDP protocols. To be specific, if we could somehow know the prior distribution of count of items and noise distribution. We can compute prosterior probability of count of each items given the output of existing LDP protocols. %However, there are several probablems we need to address. First, how to get the prior distribution of count of items? Second, how to get the probability distribution of noise? Third, how to perform posterior estimation given the observed value of each items, prior distribution as well as noise distribution.
































==> table.tex <==
\begin{table}[!t]\renewcommand{\arraystretch}{1}
\centering
\caption{Sybil classification on the Twitter dataset. Numbers in the parenthesis are standard deviations.}
\centering
%\addtolength{\tabcolsep}{-4pt}
\begin{tabular}{|c|c|c|} \hline 
{\small False Positive Categories} & {\small # of Accounts} & {\small Percentage} & {\small Notes}\\ \hline
{\small Suspended} & {\small 1} & {\small 0.99\%} & {\small Account suspended by Twitter.}\\ \hline
{\small Deteleted} & {\small 4} & {\small 3.96\%} & {\small Account deleted by user.}\\ \hline
{\small Suspicious} & {\small 1} & {\small 0.99\%} & {\small This user has another social network account. It has been suspended by the service provider. So we consider this user suspicious.}\\ \hline
{\small Commercial} & {\small 36} & {\small 35.64\%} & {\small Accounts in this category are for commercial purposes. They have hundreds of thousands of tweets, most are advertisements or links for commercial use. They tend to follow back whoever follows them. As a result, they have huge numbers of tweets, followings and followers.}\\ \hline
{\small Celebrities} & {\small 18} & {\small 17.82\%} & {\small Accounts in this category are for personal use. Most of the users are celebrities in their community. They generally have hundreds even thousands times of followers than followings.}\\ \hline
{\small Ordinary} & {\small 41} & {\small 40.59\%} & {\small Ordinary Twitter users.}\\ \hline
{\small Total} & {\small 101} & {\small 100.00\%} & {\small FNR}\\ \hline

\end{tabular}
\vspace{-4mm}
\label{falsepos}
\end{table}

